CPOT: Channel Pruning via Optimal Transport

Recent advances in deep neural networks (DNNs) lead to tremendously growing network parameters, making the deployments of DNNs on platforms with limited resources extremely difficult. Therefore, various pruning methods have been developed to compress the deep network architectures and accelerate the inference process. Most of the existing channel pruning methods discard the less important filters according to well-designed filter ranking criteria. However, due to the limited interpretability of deep learning models, designing an appropriate ranking criterion to distinguish redundant filters is difficult. To address such a challenging issue, we propose a new technique of Channel Pruning via Optimal Transport, dubbed CPOT. Specifically, we locate the Wasserstein barycenter for channels of each layer in the deep models, which is the mean of a set of probability distributions under the optimal transport metric. Then, we prune the redundant information located by Wasserstein barycenters. At last, we empirically demonstrate that, for classification tasks, CPOT outperforms the state-of-the-art methods on pruning ResNet-20, ResNet-32, ResNet-56, and ResNet-110. Furthermore, we show that the proposed CPOT technique is good at compressing the StarGAN models by pruning in the more difficult case of image-to-image translation tasks.

==> Pruning via OT/algorithm.tex <==
%%%%%%%%%%%   ALGORITHMS STYLE  %%%%%%%%%%%
% This style defines an environment for algorithms with the following
% features:
%
% 1) Defines an Theorem like environment (not exactly one) for
%    algorithms called ``algorithm''.
%    \begin{algorithm}{NAME} ... \end{algorithm}
%    NAME is the NAME of the algorithm.
%    Algorithms are numbered using a counter called ``algorithm''.
%
% 2) Inside this environment, the following commands are defined.
%
%    \=  Put the small left arrow commonly used for assignment.
%
%    \invariant{INVARIANT} Use to describe invariants, put its parameter
%                          between ``{}'' in math mode.
%
%    \begin{Block} ... \end{Block} Environment use to start a indented
%                                  block of instructions \end{Block} put
%                                  an ``end'' to close the block.
%
%    \nextBlock{SEPARATOR} Inside a Block, it allows to put a separator
%                          of parts of the indented block. Usefull for
%                          constructions like ``IF..THEN..ELSE..END''
%                       i.e. If cond then
%                            \begin{Block}
%                               then part
%                            \nextBlock{else}
%                               else part
%                            \end{Block}
%
% 3) \Blockindent and \algorithmindent are length that specify the
%    indentention of Blocks and of the algorithm resp.
%
%   4) Instructions are separated by ``\\'', ``\par'' or by leaving a
%      blank line. Before an ``\end{Block}'' a ``\\'' can't be used.
%
%
% Created by Jose Alberto Fernandez R.
% e-mail:    alberto@cs.umd.edu
%

%
\newcounter{algorithm}
\newtheorem{Alg@orithm}[algorithm]{Algorithm}
% Invariants
\newcommand{\inv@ariant}[1]{\mbox{$\{#1\}$}}
% Steps environment
\newenvironment{ste@ps}[1]{
\begin{list}{}
{\setlength\labelsep{0in}
\addtolength\partopsep\topsep
\addtolength\partopsep\parsep
\setlength\parsep{0in}
\setlength\topsep{0in}
\setlength\itemsep{0in}
\setlength\labelwidth{0in}
\setlength\rightmargin{0in}
\setlength\leftmargin{#1}}
}{
\end{list}
}

% Block environment
% Indentation of the Block
\newlength{\Blockindent}
% NextBlock command
\newcommand{\next@Block}[1]{
\end{ste@ps}
#1
\begin{ste@ps}{\Blockindent}
\item
}

\newenvironment{Blo@ck}{
\let\nextBlock\next@Block
\begin{ste@ps}{\Blockindent}
\item
}{
\end{ste@ps}
end
}
% Algorithm environment
% Assign command
\newcommand{\ass@ign}{\mbox{$\leftarrow$}}
% Indentation of the algorithm
\newlength{\algorithmindent}
% Algorithm definition
\newenvironment{algorithm}[1]{
\let\=\ass@ign
\let\invariant\inv@ariant
\let\Block\Blo@ck
\let\endBlock\endBlo@ck
\begin{Alg@orithm} #1
\rm\par
\begin{ste@ps}{\algorithmindent}
\item
}{
\end{ste@ps}
\bf end
\end{Alg@orithm}
}

% Setting default indentation
\setlength{\algorithmindent}{1em}
\setlength{\Blockindent}{2em}

% End of algorithm.sty


==> Pruning via OT/microtype.tex <==
%%
%% This is file `microtype.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% microtype.dtx  (with options: `package')
%%
%% -----------------------------------------------------------------------
%%                        The `microtype' package
%%        An interface to the micro-typographic extensions of pdfTeX
%%           Copyright (c) 2004, 2005 R Schlicht <w.m.l@gmx.net>
%%
%% This work  may be  distributed and/or modified  under the conditions of
%% the LaTeX Project Public License, either version 1.3 of this license or
%% (at your option) any later version.  The latest version of this license
%% is in:  http://www.latex-project.org/lppl.txt, and version 1.3 or later
%% is part of all distributions of LaTeX version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of the files microtype.dtx and microtype.ins and the
%% derived file microtype.sty.
%%
%% -----------------------------------------------------------------------
%%
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{microtype}
      [2005/02/02 v1.6a Micro-typography with pdfTeX (RS)]
\RequirePackage{keyval}[1997/11/10]
\def\MT@info{\PackageInfo{microtype}}
\def\MT@info@nl#1{\MT@info{#1\@gobble}}
\let\MT@vinfo\@gobble
\def\MT@warning{\PackageWarning{microtype}}
\def\MT@warning@nl#1{\MT@warning{#1\@gobble}}
\def\MT@error{\PackageError{microtype}}
\newcommand{\DeclareMicroTypeSet}[3][]{}
\newcommand{\UseMicroTypeSet}[2][]{}
\newcommand{\DeclareMicroTypeAlias}[2]{}
\newcommand{\SetProtrusion}[3][]{}
\newcommand{\SetExpansion}[3][]{}
\newcommand{\DeclareCharacterInheritance}[3][]{}
\newcommand{\microtypesetup}[1]{}
\def\DeclareMicroTypeSet{%
   \@ifstar
      {\@ifnextchar[\MT@DeclareSet{\MT@DeclareSet[]}}%
      {\@ifnextchar[\MT@DeclareSet{\MT@DeclareSet[]}}%
}
\def\MT@DeclareSet[#1]#2#3{}
\@onlypreamble{\DeclareMicroTypeSet}
\@onlypreamble{\UseMicroTypeSet}
\@onlypreamble{\DeclareMicroTypeAlias}
\let\MT@pdftex@no\z@
\ifx\pdftexversion\@undefined \else
   \ifx\pdftexversion\relax \else
      \def\MT@pdftex@no{4}
      \ifnum\pdftexversion < 120
         \let\MT@pdftex@no\thr@@
         \ifnum\pdftexversion = 14
            \ifnum \expandafter`\pdftexrevision < `h
               \let\MT@pdftex@no\tw@
            \fi
            \ifnum \expandafter`\pdftexrevision < `f
               \let\MT@pdftex@no\@ne
            \fi
         \else
            \ifnum\pdftexversion < 14
               \let\MT@pdftex@no\@ne
            \fi
         \fi
      \fi
   \fi
\fi
\let\MT@exitornot\relax
\ifnum\MT@pdftex@no<\tw@
   \def\MT@exitornot{%
      \AtEndOfPackage{\let\@unprocessedoptions\relax}%
      \let\CurrentOption\@empty
      \endinput
   }
   \MT@warning@nl{%
      \ifcase\MT@pdftex@no
         You don't seem to be using pdftex.\MessageBreak
      \or
         You are using a pdftex version older than 0.14f.\MessageBreak
         microtype doesn't support such antiquated versions.\MessageBreak
         Please install a newer version of pdftex.\MessageBreak
      \fi
         All micro-typographic features will be disabled%
   }
\fi
\MT@exitornot
\def\MT@catcodes{%
   \@makeother\-%
   \@makeother\,%
   \@makeother\/%
   \@makeother\`%
   \@makeother\'%
   \@makeother\"%
   \catcode`\^7\relax
}
\def\MT@restore@catcodes#1{%
   \ifx\relax#1\else
      \noexpand\catcode`\noexpand#1\the\catcode`#1\relax
      \expandafter\MT@restore@catcodes
   \fi
}
\edef\MT@restore@catcodes{%
   \MT@restore@catcodes\-\,\/\`\'\"\^\relax
}
\MT@catcodes
\AtEndOfPackage{\MT@restore@catcodes}
\AtBeginDocument{%
   \@ifpackageloaded{pdfcprot}{%
      \MT@error{%
         Detected the `pdfcprot' package!\MessageBreak
         `microtype' and `pdfcprot' may not be used together}%
         {The `pdfcprot' package provides an interface to
          character protrusion.\MessageBreak
          So does the `microtype' package.
          Using both packages at the same\MessageBreak
          time will almost certainly lead to undesired results.
          Have your choice!}%
   }{}%
}
\expandafter\ifx\the\font\nullfont\normalfont\fi
\newif\ifMT@DVIoutput
\newif\ifMT@draft
\newif\ifMT@protrusion
\newif\ifMT@expansion
\newif\ifMT@auto
\newif\ifMT@selected
\def\MT@expansionlevel{2}
\def\MT@protrusionlevel{2}
\let\MT@stretch\m@ne
\let\MT@shrink\m@ne
\let\MT@step\m@ne
\let\MT@prot@factor\@m
\def\MT@def@n#1{\expandafter\def\csname #1\endcsname}
\def\MT@edef@n#1{\expandafter\edef\csname #1\endcsname}
\def\MT@let@nc#1{\expandafter\let\csname #1\endcsname}
\def\MT@let@cn#1#2{\expandafter\let\expandafter#1\csname #2\endcsname}
\def\MT@hop@else@fi#1\else#2\fi{\fi#1}
\ifx\ifdefined\@undefined\MT@hop@else@fi
   \def\MT@ifdefined@c#1{%
      \ifx#1\@undefined
         \expandafter\@secondoftwo
      \else
         \expandafter\@firstoftwo
      \fi
   }
   \def\MT@ifdefined@n#1{%
      \expandafter\ifx\csname#1\endcsname\relax
         \expandafter\@secondoftwo
      \else
         \expandafter\@firstoftwo
      \fi
   }
\else
   \def\MT@ifdefined@c#1{%
      \ifdefined#1%
         \expandafter\@firstoftwo
      \else
         \expandafter\@secondoftwo
      \fi
   }
   \def\MT@ifdefined@n#1{%
      \ifcsname#1\endcsname
         \expandafter\@firstoftwo
      \else
         \expandafter\@secondoftwo
      \fi
   }
\fi
\begingroup
\catcode`\%=12\relax
\catcode`\&=14\relax
\gdef\MT@ifempty#1{&
  \if %#1%&
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}
\endgroup
\def\MT@ifnumber#1{%
   \if!\ifnum9<1#1!\else_\fi
      \expandafter\@firstoftwo
   \else
      \expandafter\@secondoftwo
   \fi
}
\def\MT@xadd#1#2{%
   \expandafter\ifx#1\relax
      \xdef#1{#2}%
   \else
      \begingroup
         \edef\x{#2}%
         \toks@=\expandafter\expandafter\expandafter{\expandafter#1\x}%
         \xdef#1{\the\toks@}%
      \endgroup
   \fi
}
\newif\ifMT@inlist@
\def\MT@in@list#1#2{%
   \MT@inlist@false
   \def\MT@given{#1}%
   \def\MT@lt##1{%
      \def\MT@next{##1}\ifx\MT@next\MT@given\MT@inlist@true\fi}#2%
}
\let\MT@lt\@empty
\def\MT@in@llist#1#2{%
   \MT@inlist@false
   \def\MT@in@l##1#1,##2\@nil{%
      \ifx\\##2\\\else
         \MT@inlist@true
      \fi}%
   \expandafter\MT@in@l#2,#1,\@nil
}
\def\MT@loop#1\MT@repeat{%
   \def\MT@iterate{#1\relax\expandafter\MT@iterate\fi}%
   \MT@iterate \let\MT@iterate\relax}
\let\MT@repeat\fi
\newcount\MT@count
\def\MT@increment#1{%
   \MT@count#1\relax
   \advance\MT@count \@ne
   \edef#1{\number\MT@count}%
}
\def\MT@remove@spaces#1{\expandafter\KV@@sp@def\expandafter#1\expandafter{#1}}
\def\MT@setupfont{%
   \ifx\MT@vinfo\MT@info@nl
      \MT@info{Setting up font `\expandafter\string\font@name'}\fi
   \expandafter\expandafter\expandafter
      \MT@split@name\expandafter\string\font@name\@nil
   \MT@find@file{\MT@family}%
   \ifx\MT@familyalias\@empty\else\MT@find@file{\MT@familyalias}\fi
   \ifx\f@encoding\cf@encoding\else\@@enc@update\fi
   \MT@checkfor{protrusion}%
   \ifMT@font@protrusion
      \MT@set@prot@codes
   \else
      \MT@vinfo{... No protrusion}%
   \fi
   \MT@checkfor{expansion}%
   \ifMT@font@expansion
      \MT@set@exp@codes
   \else
      \MT@vinfo{... No expansion}%
   \fi
}
\newif\ifMT@font@protrusion
\newif\ifMT@font@expansion
\def\MT@checkfor#1{%
   \csname ifMT@#1\endcsname
      \csname MT@font@#1true\endcsname
      \MT@checklist{#1}{encoding}%
      \MT@checklist@family{#1}%
      \MT@checklist{#1}{series}%
      \MT@checklist{#1}{shape}%
      \MT@checklist{#1}{size}%
   \fi
}
\def\MT@checklist#1#2{%
   \csname ifMT@font@#1\endcsname\MT@checklist@{#1}{#2}\fi
}
\def\MT@checklist@#1#2{%
   \edef\@tempa{\csname MT@#1@setname\endcsname}%
   \MT@ifdefined@n{MT@#1list@#2@\@tempa}{%
      \def\MT@listname{\csname MT@#1list@#2@\@tempa\endcsname}%
      \expandafter\expandafter\expandafter\MT@in@list
         \expandafter\expandafter\expandafter
            {\csname MT@#2\endcsname}\MT@listname
      \ifMT@inlist@
      \else
         \csname MT@font@#1false\endcsname
      \fi
   }{%
   }%
}
\def\MT@checklist@family#1{%
   \csname ifMT@font@#1\endcsname\MT@checklist@family@{#1}\fi
}
\def\MT@checklist@family@#1{%
   \MT@checklist@{#1}{family}%
   \csname ifMT@font@#1\endcsname\else
      \ifx\MT@familyalias\@empty\else
         \edef\@tempa{\csname MT@#1@setname\endcsname}%
         \def\MT@listname{\csname MT@#1list@family@\@tempa\endcsname}%
         \expandafter\expandafter\expandafter\MT@in@list
            \expandafter
               {\MT@familyalias}\MT@listname
         \ifMT@inlist@
            \csname MT@font@#1true\endcsname
         \fi
      \fi
   \fi
}
\def\MT@split@name#1/#2/#3/#4/#5\@nil{%
   \gdef\MT@encoding{#1}%
   \gdef\MT@family{#2}%
   \gdef\MT@series{#3}%
   \gdef\MT@shape{#4}%
   \gdef\MT@size{#5}%
   \global\let\MT@familyalias\@empty
   \MT@ifdefined@n{MT@\MT@family @alias}{%
      \MT@escapechar{\csname MT@\MT@family @alias\endcsname}%
      \global\let\MT@familyalias\MT@val
   }{}%
}
\def\MT@set@prot@codes{%
   \MT@get@codes@list{prot}%
   \MT@ifdefined@n{MT@protcodes@\MT@protcodes@name}{%
      \MT@get@factor
      \MT@get@inh@list{protrusion}%
      \MT@ifdefined@c\MT@protrusioninh@name{%
         \MT@let@cn\@tempc{MT@protrusioninh@\MT@protrusioninh@name}%
            \ifx\@tempc\@empty\else
               \let\MT@inh@name\MT@protrusioninh@name
               \expandafter\MT@inhdo\@tempc,\relax,%
            \fi
         \global\MT@let@nc{MT@protrusioninh@\MT@protrusioninh@name}\@empty
      }{}%
      \MT@load@list{prot}{\MT@protcodes@name}%
      \MT@let@cn\@tempc{MT@protcodes@\MT@protcodes@name}%
      \expandafter\MT@protdo\@tempc,\relax,%
   }{}%
}
\def\MT@protdo#1,{%
   \ifx\relax#1\@empty\else
      \MT@protsplit #1==\relax
      \expandafter\MT@protdo\fi
}
\def\MT@protsplit#1=#2=#3\relax{%
   \KV@@sp@def\@tempa{#1}%
   \ifx\@tempa\@empty\else
      \MT@get@slot
      \ifnum\MT@char > \m@ne
         \KV@@sp@def\@tempb{#2}%
         \expandafter\MT@protsplit@val\@tempb\relax
      \fi
   \fi
}
\def\MT@protsplit@val#1,#2\relax{%
   \KV@@sp@def\@tempb{#1}%
   \MT@ifempty{\@tempb}{}{%
      \MT@adjustprotcode
      \lpcode\font@name\MT@char=\@tempcntb
   }%
   \KV@@sp@def\@tempb{#2}%
   \MT@ifempty{\@tempb}{}{%
      \MT@adjustprotcode
      \rpcode\font@name\MT@char=\@tempcntb
   }%
   \MT@ifdefined@c\MT@protrusioninh@name{%
      \MT@ifdefined@n{MT@inh@\MT@protrusioninh@name @\MT@char @}{%
         \MT@set@prot@children
      }{}%
   }{}%
}
\ifnum\MT@pdftex@no>\tw@
   \def\MT@adjustprotcode{%
      \MT@get@charwd
      \multiply\@tempcntb \@tempb
      \ifnum\@tempcntb=\z@ \else
         \divide\@tempcntb \fontdimen6 \font@name
         \MT@adjustprotcode@
      \fi
   }
   \MT@ifdefined@c\fontcharwd{%
      \def\MT@get@charwd{%
         \@tempcntb=\number\fontcharwd\font@name\MT@char}%
   }{%
      \def\MT@get@charwd{%
         \setbox\z@=\hbox{\font@name \char\MT@char}%
         \@tempcntb=\wd\z@}%
   }
\else
   \def\MT@adjustprotcode{%
      \@tempcntb=\@tempb
      \ifnum\@tempcntb=\z@ \else
         \MT@adjustprotcode@
      \fi
   }
\fi
\def\MT@adjustprotcode@{%
   \multiply\@tempcntb \MT@prot@factor@
   \divide\@tempcntb \@m
   \ifnum\@tempcntb > \@m
      \MT@warning@nl{Protrusion factor \@tempb\space for character
         `\@tempa'\MessageBreak too large (= \the\@tempcntb) in
         protrusion list `\MT@protcodes@name'}%
   \else
      \ifnum\@tempcntb < -\@m
         \MT@warning@nl{Protrusion factor \@tempb\space for character
            `\@tempa'\MessageBreak too small (= \the\@tempcntb) in
            protrusion list `\MT@protcodes@name'}%
      \fi
   \fi
}
\def\MT@set@prot@children{%
   \def\MT@lt##1{%
      \lpcode\font@name##1=\lpcode\font@name\MT@char
      \rpcode\font@name##1=\rpcode\font@name\MT@char
   }%
   \csname MT@inh@\MT@protrusioninh@name @\MT@char @\endcsname
}
\def\MT@get@factor{%
   \MT@ifdefined@n{MT@protcodes@\MT@protcodes@name @factor}{%
      \MT@let@cn\MT@prot@factor@{MT@protcodes@\MT@protcodes@name @factor}%
      \MT@vinfo{... ... Multiplying protrusion factors by \MT@prot@factor@/1000}%
   }{%
      \let\MT@prot@factor@\MT@prot@factor
   }%
}
\newif\ifMT@selected@exp
\def\MT@set@exp@codes{%
   \ifMT@selected
      \MT@get@codes@list{exp}%
      \MT@ifdefined@n{MT@expcodes@\MT@expcodes@name}{%
         \MT@get@extraopt
         \MT@resetefcode
         \MT@get@inh@list{expansion}%
         \MT@ifdefined@c\MT@expansioninh@name{%
            \MT@let@cn\@tempc{MT@expansioninh@\MT@expansioninh@name}%
               \ifx\@tempc\@empty\else
                  \let\MT@inh@name\MT@expansioninh@name
                  \expandafter\MT@inhdo\@tempc,\relax,%
               \fi
            \global\MT@let@nc{MT@expansioninh@\MT@expansioninh@name}\@empty
         }{}%
         \MT@load@list{exp}{\MT@expcodes@name}%
         \MT@let@cn\@tempc{MT@expcodes@\MT@expcodes@name}%
         \expandafter\MT@expdo\@tempc,\relax,%
         \pdffontexpand\font@name \MT@stretch@ \MT@shrink@ \MT@step@ \MT@auto@
      }{}%
   \else
      \MT@selected@exptrue
      \MT@get@codes@list{exp}%
      \MT@ifdefined@n{MT@expcodes@\MT@expcodes@name}{%
         \MT@get@extraopt
      }{%
         \let\MT@exp@factor@\@m
         \let\MT@stretch@\MT@stretch
         \let\MT@shrink@\MT@shrink
         \let\MT@step@\MT@step
         \let\MT@auto@\MT@auto
      }%
      \MT@resetefcode
      \pdffontexpand\font@name \MT@stretch@ \MT@shrink@ \MT@step@ \MT@auto@
   \fi
}
\def\MT@resetefcode@{%
   \@tempcnta\z@
   \MT@loop
      \efcode\font@name\@tempcnta=\MT@exp@factor@
      \advance\@tempcnta \@ne
      \ifnum\@tempcnta < \@cclvi \MT@repeat
}
\ifnum\MT@pdftex@no<4
   \let\MT@resetefcode\MT@resetefcode@
\else
   \def\MT@resetefcode{%
      \ifnum\MT@exp@factor@=\@m \else
         \MT@resetefcode@
      \fi
   }
\fi
\def\MT@expdo#1,{%
   \ifx\relax#1\@empty\else
      \MT@expsplit #1==\relax
      \expandafter\MT@expdo\fi
}
\def\MT@expsplit#1=#2=#3\relax{%
   \KV@@sp@def\@tempa{#1}%
   \ifx\@tempa\@empty\else
      \MT@get@slot
      \ifnum\MT@char > \m@ne
         \KV@@sp@def\@tempb{#2}%
         \@tempcnta=\@tempb
         \multiply\@tempcnta \MT@exp@factor@
         \divide\@tempcnta \@m
         \efcode\font@name\MT@char=\@tempcnta
         \MT@ifdefined@c\MT@expansioninh@name{%
            \MT@ifdefined@n{MT@inh@\MT@expansioninh@name @\MT@char @}%
               {\MT@set@exp@children}{}%
         }{}%
      \fi
   \fi
}
\def\MT@set@exp@children{%
   \def\MT@lt##1{%
      \efcode\font@name##1=\efcode\font@name\MT@char
   }%
   \csname MT@inh@\MT@expansioninh@name @\MT@char @\endcsname
}
\def\MT@get@extraopt{%
   \MT@ifdefined@n{MT@expcodes@\MT@expcodes@name @factor}{%
      \MT@let@cn\MT@exp@factor@{MT@expcodes@\MT@expcodes@name @factor}%
      \MT@vinfo{... ... Multiplying expansion factors by \MT@exp@factor@/1000}%
   }{%
      \let\MT@exp@factor@\@m
   }%
   \MT@ifdefined@n{MT@expcodes@\MT@expcodes@name @stretch}{%
      \MT@let@cn\MT@stretch@{MT@expcodes@\MT@expcodes@name @stretch}%
      \MT@vinfo{... ... Setting stretch factor to \MT@stretch@}%
   }{%
      \let\MT@stretch@\MT@stretch
   }%
   \MT@ifdefined@n{MT@expcodes@\MT@expcodes@name @shrink}{%
      \MT@let@cn\MT@shrink@{MT@expcodes@\MT@expcodes@name @shrink}%
      \MT@vinfo{... ... Setting shrink factor to \MT@shrink@}%
   }{%
      \let\MT@shrink@\MT@shrink
   }%
   \MT@ifdefined@n{MT@expcodes@\MT@expcodes@name @step}{%
      \MT@let@cn\MT@step@{MT@expcodes@\MT@expcodes@name @step}%
      \MT@vinfo{... ... Setting step factor to \MT@step@}%
   }{%
      \let\MT@step@\MT@step
   }%
   \MT@ifdefined@n{MT@expcodes@\MT@expcodes@name @auto}{%
      \MT@let@cn\MT@auto@{MT@expcodes@\MT@expcodes@name @auto}%
      \MT@vinfo{... ... Setting automatic expansion to \MT@auto@}%
   }{%
      \let\MT@auto@\MT@auto
   }%
}
\def\MT@load@list#1#2{%
   \edef\@tempa{#2}%
   \MT@let@cn\@tempb{MT@#1codes@\@tempa load}%
   \ifx\@tempa\@tempb
      \MT@warning{#1. list `\@tempa' cannot load itself}%
   \else
      \ifx\@tempb\relax\else
         \MT@ifdefined@n{MT@#1codes@\@tempb}{%
            \MT@vinfo{... ... Additionally loading #1. list `\@tempb'}%
            \begingroup
               \MT@load@list{#1}{\@tempb}%
            \endgroup
            \MT@let@cn\@tempc{MT@#1codes@\@tempb}%
            \expandafter\csname MT@#1do\expandafter\endcsname\@tempc,\relax,%
         }{%
            \MT@warning{%
               #1. list `\@tempb' undefined. Cannot load it\MessageBreak
               from list `\@tempa'}%
         }%
      \fi
   \fi
}
\let\MT@file@list\@empty
\def\MT@find@file#1{%
   \expandafter\MT@in@llist\expandafter
         {\csname MT@file@#1\endcsname}\MT@file@list
   \ifMT@inlist@\else
      \begingroup
      \MT@file@catcodes
      \InputIfFileExists{mt-#1.cfg}{%
         \MT@xadd\MT@file@list{\csname MT@file@#1\endcsname,}%
         \MT@vinfo{... Loading font settings from mt-#1.cfg}%
      }{%
         \expandafter\MT@get@basefamily#1\relax\relax\relax
         \expandafter\MT@in@llist\expandafter
                {\csname MT@file@\@tempa\endcsname}\MT@file@list
         \ifMT@inlist@\else
            \InputIfFileExists{mt-\@tempa.cfg}{%
               \MT@xadd\MT@file@list{\csname MT@file@\@tempa\endcsname,}%
               \MT@vinfo{... Loading font settings from mt-\@tempa.cfg}%
            }{%
               \MT@xadd\MT@file@list{\csname MT@file@#1\endcsname,}%
               \MT@vinfo{... No file mt-#1.cfg}%
            }%
         \fi
      }%
      \endgroup
   \fi
}
\def\MT@file@catcodes{%
     \makeatletter
     \catcode`\ 9%
     \catcode`\^7%
     \catcode`\^^I9%
     \catcode`\^^M9%
     \catcode`\\\z@
     \catcode`\{\@ne
     \catcode`\}\tw@
     \catcode`\#6%
     \catcode`\%14%
   \@makeother\<%
   \@makeother\>%
   \@makeother\*%
   \@makeother\.%
   \@makeother\-%
   \@makeother\/%
   \@makeother\[%
   \@makeother\]%
   \@makeother\`%
   \@makeother\'%
   \@makeother\"%
   \@makeother\&%
   \@makeother\;%
   \@makeother\,%
   \@makeother\!%
   \@makeother\?%
   \@makeother\$%
   \@makeother\_%
   \@makeother\~%
   \@makeother\=%
}
\def\MT@get@basefamily#1#2#3#4\relax{%
   \ifx\relax#2\relax\def\@tempa{#1}\else
      \ifx\relax#3\relax\def\@tempa{#1#2}\else
         \def\@tempa{#1#2#3}%
         \ifx\relax#4\relax\else
            \edef\@tempc{\string#4}%
            \edef\@tempb{\string x}%
            \ifx\@tempc\@tempb\else
               \edef\@tempb{\string j}%
               \ifx\@tempc\@tempb\else
                  \edef\@tempb{\string w}%
                  \ifx\@tempc\@tempb\else
                     \def\@tempa{#1#2#3#4}%
                  \fi
               \fi
            \fi
         \fi
      \fi
   \fi
}
\def\MT@get@listname#1{%
   \def\@tempb{#1}%
   \MT@next@listname1111\relax
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \MT@next@listname1110\relax
   }%
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \MT@next@listname1100\relax
   }%
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \MT@next@listname1010\relax
   }%
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \MT@next@listname1000\relax
   }%
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \MT@next@listname0100\relax
   }%
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \MT@next@listname0010\relax
   }%
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \MT@next@listname0000\relax
   }%
}
\def\MT@next@listname#1#2#3#4{%
   \edef\@tempa{\MT@encoding/%
                \ifnum#1=\@ne \MT@family\fi/%
                \ifnum#2=\@ne \MT@series\fi/%
                \ifnum#3=\@ne \MT@shape\fi/%
                \ifnum#4=\@ne \MT@size\fi}%
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \ifnum#1=\@ne
         \ifx\MT@familyalias\@empty\else
            \edef\@tempa{\MT@encoding/%
                         \MT@familyalias/%
                         \ifnum#2=\@ne \MT@series\fi/%
                         \ifnum#3=\@ne \MT@shape\fi/%
                         \ifnum#4=\@ne \MT@size\fi}%
         \fi
      \fi
   }%
}
\def\MT@get@codes@list#1{%
   \MT@get@listname{#1codes}%
   \MT@ifdefined@n{MT@#1codes@\@tempa}{%
      \global\MT@edef@n{MT@#1codes@name}{\csname MT@#1codes@\@tempa\endcsname}%
      \ifMT@selected@exp
         \MT@vinfo{... Applying non-selected expansion (list `\MT@expcodes@name')}%
      \else
         \MT@vinfo{... Using #1. list `\csname MT@#1codes@name\endcsname'}%
      \fi
   }{%
      \global\MT@let@nc{MT@#1codes@\csname MT@#1codes@name\endcsname}\@undefined
      \ifMT@selected@exp
         \MT@vinfo{... Applying non-selected expansion}%
      \else
         \MT@warning{I cannot find a #1. list for
                     `\expandafter\string\font@name'.\MessageBreak
                     Switching off #1. for this font}%
       \fi
   }%
}
\def\MT@get@inh@list#1{%
   \MT@get@listname{#1inh}%
   \MT@ifdefined@n{MT@#1inh@\@tempa}{%
      \MT@edef@n{MT@#1inh@name}{\csname MT@#1inh@\@tempa\endcsname}%
   }{%
      \MT@let@nc{MT@#1inh@name}\@undefined
   }%
}
\begingroup
   \catcode`\/=0
   /catcode`/\=12
   /catcode`/"=12
   /catcode`/A=12
   /catcode`/C=12
   /catcode`/E=12
   /catcode`/H=12
   /catcode`/L=12
   /catcode`/R=12
   /catcode`/T=12
   /lowercase{%
      /def/x{%
         /def/Mt@letterstring{THE LETTER}%
         /def/Mt@isaletter ##1THE LETTER##2##3/relax{%
            /@tempswafalse
            /ifx/relax##1/relax
               /@tempswatrue
               /edef/Mt@char{/number`##2}%
               /Mt@testrest{/Mt@letterstring}{##3}%
            /fi
         }%
         /def/Mt@characterstring{THE CHARACTER}%
         /def/Mt@isacharacter ##1THE CHARACTER##2##3/relax{%
            /@tempswafalse
            /ifx/relax##1/relax
               /@tempswatrue
               /edef/Mt@char{/number`##2}%
               /Mt@testrest{/Mt@characterstring}{##3}%
            /fi
         }%
         /def/Mt@charstring{\CHAR"}%
         /def/Mt@isachar##1\CHAR"##2##3##4/relax{%
            /@tempswafalse
            /ifx/relax##1/relax
               /@tempswatrue
               /if##3\/relax
                  /edef/Mt@char{/number"##2}%
                  /Mt@testrest{/Mt@charstring}{##3##4}%
               /else
                  /edef/Mt@char{/number"##2##3}%
                  /Mt@testrest{/Mt@charstring}{##4}%
               /fi
            /fi
         }%
      }%
   }
/expandafter/endgroup/x
\def\Mt@testrest#1#2{%
   \edef\x{#1}%
   \edef\y{#2}%
   \ifx\x\y\else
      \def\Mt@rest{#2}%
   \fi
}
\def\MT@get@slot{%
   \MT@count=\escapechar
   \escapechar=`\\
   \let\Mt@rest\@empty
   \let\Mt@char\m@ne
   \edef\MT@char{\expandafter\meaning\@tempa}%
   \expandafter\expandafter\expandafter\Mt@isaletter
         \expandafter\MT@char\Mt@letterstring \relax\relax
   \ifnum\Mt@char < \z@
      \expandafter\expandafter\expandafter\Mt@isacharacter
            \expandafter\MT@char\Mt@characterstring \relax\relax
      \if@tempswa
         \expandafter\MT@get@number\@tempa\relax\relax
      \fi
      \ifnum\Mt@char < \z@
         \expandafter\ifx\expandafter\ \@tempa\relax
            \edef\Mt@char{\number`\\}%
         \else
            \edef\MT@char{\expandafter\csname\expandafter\MT@encoding
                              \expandafter\string\@tempa\endcsname}%
            \edef\MT@char{\expandafter\meaning\MT@char}%
            \expandafter\expandafter\expandafter\Mt@isachar
                  \expandafter\MT@char\Mt@charstring \relax\relax\relax
            \if@tempswa \else
               \expandafter\expandafter\expandafter\Mt@isaletter
                     \expandafter\MT@char\Mt@letterstring \relax\relax
            \fi
         \fi
         \ifnum\Mt@char < \z@
            \expandafter\MT@two@tokens\@tempa\relax\relax
            \edef\MT@char{\expandafter\meaning\@tempa}%
            \expandafter\expandafter\expandafter\Mt@isaletter
                  \expandafter\MT@char\Mt@letterstring \relax\relax
            \if@tempswa \else
               \MT@warning{Unknown slot number of `\@tempa' in\MessageBreak
                           encoding `\MT@encoding'. Ignoring it}%
            \fi
         \fi
      \fi
   \fi
   \ifx\Mt@rest\@empty\else
      \MT@warning{Unknown slot number of `\@tempa' in\MessageBreak
                  encoding `\MT@encoding'.
                  Make sure it's a single character\MessageBreak
                  (or a number). Ignoring it}%
      \let\Mt@char\m@ne
   \fi
   \let\MT@char\Mt@char
   \escapechar=\MT@count
}
\def\MT@two@tokens#1#2\relax{%
   \MT@ifempty{#2}{}%
      {\edef\@tempa{\@tempa}}%
}
\def\MT@get@number#1#2#3\relax{%
   \ifx\relax#3\relax\else
      \ifx\relax#2\relax\else
         \if#1"\relax
            \def\@tempc{\uppercase{\edef\Mt@char{\number#1#2#3}}}%
            \@tempc
         \else
            \if#1'\relax
               \def\Mt@char{\number#1#2#3}%
            \else
               \MT@ifnumber{#1#2#3}{%
                  \def\Mt@char{\number#1#2#3}%
               }{}%
            \fi
         \fi
         \ifnum\Mt@char > \@cclv
            \MT@warning{%
               Number \noexpand#1\noexpand#2\noexpand#3 in encoding
               `\MT@encoding' too large!\MessageBreak Ignoring it}%
            \let\Mt@char\m@ne
         \fi
         \let\Mt@rest\@empty
      \fi
   \fi
}
\let\MT@font@list\@empty
\g@addto@macro\pickup@font{%
   \begingroup \escapechar\m@ne
   \expandafter\MT@in@llist\expandafter
         {\font@name}\MT@font@list
   \ifMT@inlist@\else
      \MT@setupfont
      \xdef\MT@font@list{\MT@font@list\font@name,}%
   \fi
   \endgroup
}
\let\MT@pickupfont\pickup@font
\AtBeginDocument{%
   \ifx\MT@pickupfont\pickup@font\else
      \MT@warning@nl{%
         Another package has overwritten the definition\MessageBreak
         of \string\pickup@font. I might not be able to\MessageBreak
         apply any micro-typography. Please find the\MessageBreak
         culprit, and load it before the microtype package}%
   \fi
}
\def\DeclareMicroTypeSet{%
   \@ifstar
      {\@ifnextchar[%]
         \MT@DeclareSetAndUseIt
         {\MT@DeclareSetAndUseIt[]}}%
      {\@ifnextchar[%]
         \MT@DeclareSet
         {\MT@DeclareSet[]}}%
}
\def\MT@DeclareSet[#1]#2#3{%
   \MT@DeclareSet@{#1}{#2}{#3}%
}
\def\MT@DeclareSetAndUseIt[#1]#2#3{%
   \MT@DeclareSet@{#1}{#2}{#3}%
   \UseMicroTypeSet[#1]{#2}%
}
\def\MT@DeclareSet@#1#2#3{%
  \KV@@sp@def\@tempa{#1}%
  \MT@ifempty{\@tempa}{%
     \MT@declare@sets{protrusion}{#2}{#3}%
     \MT@declare@sets{expansion} {#2}{#3}%
  }{%
     \expandafter\MT@declare@sets\expandafter{\@tempa}{#2}{#3}%
  }%
}
\let\MT@tmp@setname\@empty
\def\MT@declare@sets#1#2#3{%
   \KV@@sp@def\MT@tmp@setname{#2}%
   \global\MT@let@nc{MT@#1list@@\MT@tmp@setname}\@empty
   \setkeys{MT#1@set}{#3}%
}
\def\MT@define@set@keys#1{%
   \MT@define@set@key{#1}{encoding}%
   \MT@define@set@key{#1}{family}%
   \MT@define@set@key{#1}{series}%
   \MT@define@set@key{#1}{shape}%
   \MT@define@set@key@size{#1}%
}
\def\MT@define@set@key#1#2{%
   \define@key{MT#1@set}{#2}[]{%
      \@for\MT@val:=##1\do{%
         \MT@remove@spaces{\MT@val}%
         \MT@get@highlevel{#2}%
         \MT@escapechar{\MT@val}%
         \MT@addto@list{#1}{#2}{\MT@val}%
      }%
   }%
}
\def\MT@get@highlevel#1{%
   \MT@getlast{\MT@val}%
   \if*\@tempb
      \MT@ifempty{\@tempa}{\def\@tempa{#1}}{}%
      \def\MT@val{\csname \@tempa default\endcsname}%
      \ifx\@nodocument\relax\else
         \expandafter\ifx
               \csname MT@check@\MT@tmp@setname @\@tempa\endcsname\@empty
         \else
            \global\MT@edef@n{MT@\MT@tmp@setname @\@tempa @default}{\MT@val}%
            \edef\x{{\MT@tmp@setname}{\@tempa}}%
            \expandafter\AtBeginDocument\expandafter{%
               \expandafter\MT@check@default\x
            }%
            \global\MT@let@nc{MT@check@\MT@tmp@setname @\@tempa}\@empty
         \fi
      \fi
   \fi
}
\def\MT@check@default#1#2{%
   \MT@let@cn\@tempa{MT@#1@#2@default}%
   \edef\@tempb{\csname #2default\endcsname}%
   \ifx\@tempa\@tempb\else
      \MT@warning@nl{\expandafter\noexpand\csname #2default\endcsname
            has changed (`\@tempa' <> `\@tempb')!\MessageBreak
            This might affect the `#1' font set.\MessageBreak
            Please make all relevant font changes *before*\MessageBreak
            loading the `microtype' package}%
   \fi
}
\def\MT@getlast#1{\def\@tempa{}\def\@tempb{}%
   \expandafter\MT@getlast@#1\@nil}
\def\MT@getlast@#1{\ifx#1\@nil \let\next=\relax
   \else \edef\@tempa{\@tempa\@tempb}\def\@tempb{#1}%
      \let\next=\MT@getlast@\fi \next}
\def\MT@escapechar#1{%
   \begingroup
   \escapechar\m@ne
   \xdef\MT@val{\expandafter\string\csname #1\endcsname}%
   \endgroup
}
\def\MT@define@set@key@size#1{%
   \define@key{MT#1@set}{size}[]{%
      \@for\MT@val:=##1\do{%
         \MT@remove@spaces{\MT@val}%
         \MT@get@size
         \MT@addto@list{#1}{size}{\MT@val}%
      }%
   }%
}
\def\MT@get@size{%
   \let\@tempa\relax
   \if*\MT@val\relax
      \def\@tempa{\normalsize}%
   \else
      \MT@let@cn\@tempa{\MT@val}%
   \fi
   \ifx\@tempa\relax\else
      \begingroup
         \def\set@fontsize##1##2##3##4\@nil{\gdef\MT@val{##2}}%
         \@tempa\@nil
      \endgroup
   \fi
   \setbox\z@=\hbox{\MT@count=0\MT@val\relax
      \ifnum\MT@count=\z@
         \@tempswafalse
      \else
         \@tempswatrue
      \fi\expandafter}%
   \if@tempswa
      \@defaultunits\@tempdima\MT@val pt\relax\@nnil
      \edef\MT@val{\strip@pt\@tempdima}%
   \else
      \MT@warning{Could not parse font size `\MT@val'\MessageBreak
                  in font set `\MT@tmp@setname'}%
   \fi
}
\def\MT@addto@list#1#2#3{%
   \expandafter\MT@xadd\csname MT@#1list@#2@\MT@tmp@setname\endcsname
      {\noexpand\MT@lt{#3}}%
}
\MT@define@set@keys{protrusion}
\MT@define@set@keys{expansion}
\renewcommand{\UseMicroTypeSet}[2][]{%
   \KV@@sp@def\@tempa{#1}%
   \MT@ifempty{\@tempa}{%
      \MT@use@sets{protrusion}{#2}%
      \MT@use@sets{expansion} {#2}%
   }{%
      \expandafter\MT@use@sets\expandafter{\@tempa}{#2}%
   }%
}
\def\MT@use@sets#1#2{%
   \KV@@sp@def{\@tempa}{#2}%
   \MT@ifdefined@n{MT@#1list@@\@tempa}{%
      \global\MT@edef@n{MT@#1@setname}{\@tempa}%
      \MT@info{Using #1 set `\@tempa'}%
   }{%
      \MT@ifdefined@n{MT@#1@setname}{}{%
         \global\MT@def@n{MT@#1@setname}{alltext}%
      }%
      \MT@warning{The #1 set `\@tempa' is undeclared.\MessageBreak
                  Using set `\csname MT@#1@setname\endcsname' instead}%
   }%
}
\renewcommand{\DeclareMicroTypeAlias}[2]{%
   \KV@@sp@def\@tempa{#1}%
   \KV@@sp@def\@tempb{#2}%
   \global\MT@edef@n{MT@\@tempa @alias}{\@tempb}%
}
\renewcommand{\SetProtrusion}[3][]{%
   \global\let\MT@protcodes@name\@undefined
   \let\MT@load\@undefined
   \let\MT@extra@factor\@undefined
   \setkeys{MT@protcodes}{#1}%
   \MT@get@codes@name{prot}%
   \MT@set@factor
   \global\MT@def@n{MT@protcodes@\MT@protcodes@name}{#3}%
   \setkeys{MT@protcodes}{#2}%
   \def\MT@permutelist{protcodes}%
   \MT@permute
}
\renewcommand{\SetExpansion}[3][]{%
   \global\let\MT@expcodes@name\@undefined
   \let\MT@extra@factor\@undefined
   \let\MT@extra@stretch\@undefined
   \let\MT@extra@shrink\@undefined
   \let\MT@extra@step\@undefined
   \let\MT@extra@auto\@undefined
   \let\MT@load\@undefined
   \setkeys{MT@expcodes}{#1}%
   \MT@get@codes@name{exp}%
   \MT@set@exp@opt
   \global\MT@def@n{MT@expcodes@\MT@expcodes@name}{#3}%
   \setkeys{MT@expcodes}{#2}%
   \def\MT@permutelist{expcodes}%
   \MT@permute
}
\def\MT@get@codes@name#1{%
   \MT@ifdefined@n{MT@#1codes@name}{%
      \MT@ifdefined@n{MT@#1codes@\csname MT@#1codes@name\endcsname}{%
         \MT@warning{Redefining list `\csname MT@#1codes@name\endcsname'}%
      }{}%
   }{%
      \@tempcnta=\@ne
      \MT@loop
         \MT@ifdefined@n{MT@#1codes@#1-\romannumeral\@tempcnta}{%
            \advance \@tempcnta \@ne
         }{%
            \global\MT@edef@n{MT@#1codes@name}{#1-\romannumeral\@tempcnta}%
            \@tempcnta=\z@
         }%
         \ifnum\@tempcnta > \z@ \MT@repeat
   }%
   \MT@ifdefined@c\MT@load{%
      \global\MT@let@nc{MT@#1codes@\csname MT@#1codes@name\endcsname load}\MT@load
   }{}%
}
\def\MT@set@factor{%
   \MT@ifdefined@c\MT@extra@factor{%
      \global\MT@let@nc{MT@protcodes@\MT@protcodes@name @factor}\MT@extra@factor
   }{}%
}
\def\MT@set@exp@opt{%
   \MT@ifdefined@c\MT@extra@factor{%
      \global\MT@let@nc{MT@expcodes@\MT@expcodes@name @factor}\MT@extra@factor
   }{}%
   \MT@ifdefined@c\MT@extra@stretch{%
      \global\MT@let@nc{MT@expcodes@\MT@expcodes@name @stretch}\MT@extra@stretch
   }{}%
   \MT@ifdefined@c\MT@extra@shrink{%
      \global\MT@let@nc{MT@expcodes@\MT@expcodes@name @shrink}\MT@extra@shrink
   }{}%
   \MT@ifdefined@c\MT@extra@step{%
      \global\MT@let@nc{MT@expcodes@\MT@expcodes@name @step}\MT@extra@step
   }{}%
   \MT@ifdefined@c\MT@extra@auto{%
      \global\MT@let@nc{MT@expcodes@\MT@expcodes@name @auto}\MT@extra@auto
   }{}%
}
\def\MT@define@code@key#1#2{%
   \define@key{MT@#1}{#2}[]{%
      \@tempcnta=\@ne
      \@for\MT@val:=##1\do{%
         \MT@remove@spaces{\MT@val}%
         \MT@get@highlevel{#2}%
         \MT@edef@n{MT@temp#2\romannumeral\@tempcnta}{\MT@val}%
         \advance\@tempcnta \@ne
      }%
   }%
}
\def\MT@define@code@key@size#1{%
   \define@key{MT@#1}{size}[]{%
      \@tempcnta=\@ne
      \@for\MT@val:=##1\do{%
         \MT@remove@spaces{\MT@val}%
         \MT@get@size
         \MT@edef@n{MT@tempsize\romannumeral\@tempcnta}{\MT@val}%
         \advance\@tempcnta \@ne
      }%
   }%
}
\def\MT@declare@codes#1{%
   \define@key{MT@#1codes}{name}[]{%
      \MT@ifempty{##1}{}{%
         \global\MT@def@n{MT@#1codes@name}{##1}%
      }%
   }%
   \define@key{MT@#1codes}{load}[]{%
      \MT@ifempty{##1}{}{%
         \def\MT@load{##1}%
      }%
   }%
   \define@key{MT@#1codes}{factor}[]{%
      \MT@ifempty{##1}{}{%
         \def\MT@extra@factor{##1 }%
      }%
   }%
   \MT@define@code@key{#1codes}{encoding}%
   \MT@define@code@key{#1codes}{family}%
   \MT@define@code@key{#1codes}{series}%
   \MT@define@code@key{#1codes}{shape}%
   \MT@define@code@key@size{#1codes}%
}
\MT@declare@codes{prot}
\MT@declare@codes{exp}
\def\MT@define@expcodes@key#1{%
   \define@key{MT@expcodes}{#1}[]{%
      \MT@ifempty{##1}{}{%
         \MT@def@n{MT@extra@#1}{##1 }%
      }%
   }%
}
\MT@define@expcodes@key{stretch}
\MT@define@expcodes@key{shrink}
\MT@define@expcodes@key{step}
\define@key{MT@expcodes}{auto}[]{%
   \MT@ifempty{#1}{\def\@tempb{true}}{\def\@tempb{#1}}%
   \csname if\@tempb\endcsname
      \def\MT@extra@auto{autoexpand }%
   \else
      \let\MT@extra@auto\@empty
   \fi
}
\renewcommand{\DeclareCharacterInheritance}[3][]{%
   \KV@@sp@def\@tempa{#1}%
   \MT@ifempty{\@tempa}{%
       \MT@declare@char@inh{protrusion}{#2}{#3}%
       \MT@declare@char@inh{expansion} {#2}{#3}%
   }{%
       \expandafter\MT@declare@char@inh\expandafter{\@tempa}{#2}{#3}%
   }%
}
\def\MT@declare@char@inh#1#2#3{%
   \MT@let@nc{MT@#1inh@name}\@undefined
   \MT@get@inh@name{#1}%
   \global\MT@def@n{MT@#1inh@\csname MT@#1inh@name\endcsname}{#3}%
   \setkeys{MT@#1inh}{#2}%
   \def\MT@permutelist{#1inh}%
   \MT@permute
}
\def\MT@get@inh@name#1{%
   \@tempcnta=\@ne
   \MT@loop
      \MT@ifdefined@n{MT@#1inh@#1-inh-\romannumeral\@tempcnta}{%
         \advance \@tempcnta \@ne
      }{%
         \MT@edef@n{MT@#1inh@name}{#1-inh-\romannumeral\@tempcnta}%
         \@tempcnta=\z@
      }%
      \ifnum\@tempcnta > \z@ \MT@repeat
}
\def\MT@define@inh@key@encoding#1{%
   \define@key{MT@#1}{encoding}[]{%
      \KV@@sp@def\MT@val{##1}%
      \expandafter\MT@encoding@check\MT@val,\@nil
      \MT@get@highlevel{encoding}%
      \MT@edef@n{MT@tempencoding\romannumeral1}{\MT@val}%
   }%
}
\def\MT@encoding@check#1,#2\@nil{%
   \MT@ifempty{#2}{}{%
      \edef\MT@val{#1}%
      \MT@warning{You may only specify one encoding for character\MessageBreak
                  inheritance lists. Ignoring encoding #2}%
   }%
}
\def\MT@define@inh@keys#1{%
   \MT@define@inh@key@encoding{#1inh}%
   \MT@define@code@key{#1inh}{family}%
   \MT@define@code@key{#1inh}{series}%
   \MT@define@code@key{#1inh}{shape}%
   \MT@define@code@key@size{#1inh}%
}
\MT@define@inh@keys{protrusion}
\MT@define@inh@keys{expansion}
\def\MT@inhdo#1,{%
   \ifx\relax#1\@empty\else
      \MT@inhsplit #1==\relax
      \expandafter\MT@inhdo\fi
}
\def\MT@inhsplit#1=#2=#3\relax{%
   \KV@@sp@def\@tempa{#1}%
   \ifx\@tempa\@empty\else
      \MT@get@slot
      \ifnum\MT@char > \m@ne
         \let\MT@val\MT@char
         \let\MT@lt\relax
         \KV@@sp@def\@tempb{#2}%
         \@for\@tempa:=\@tempb\do{%
            \MT@remove@spaces{\@tempa}%
            \ifx\@tempa\@empty\else
               \MT@get@slot
               \ifnum\MT@char > \m@ne
                  \expandafter\MT@xadd\csname MT@inh@\MT@inh@name @\MT@val @\endcsname
                     {\noexpand\MT@lt{\MT@char}}%
               \fi
            \fi
         }%
      \fi
   \fi
}
\def\MT@permute{%
   \let\MT@cnt@encoding\@ne
   \MT@permute@
   \MT@permute@reset
}
\def\MT@permute@{%
   \let\MT@cnt@family\@ne
   \MT@permute@@
   \MT@increment\MT@cnt@encoding
   \MT@ifdefined@n{MT@tempencoding\romannumeral\MT@cnt@encoding}%
      {\MT@permute@}{}%
}
\def\MT@permute@@{%
   \let\MT@cnt@series\@ne
   \MT@permute@@@
   \MT@increment\MT@cnt@family
   \MT@ifdefined@n{MT@tempfamily\romannumeral\MT@cnt@family}%
      {\MT@permute@@}{}%
}
\def\MT@permute@@@{%
   \let\MT@cnt@shape\@ne
   \MT@permute@@@@
   \MT@increment\MT@cnt@series
   \MT@ifdefined@n{MT@tempseries\romannumeral\MT@cnt@series}%
      {\MT@permute@@@}{}%
}
\def\MT@permute@@@@{%
   \let\MT@cnt@size\@ne
   \MT@permute@@@@@
   \MT@increment\MT@cnt@shape
   \MT@ifdefined@n{MT@tempshape\romannumeral\MT@cnt@shape}%
      {\MT@permute@@@@}{}%
}
\def\MT@permute@@@@@{%
   \MT@permute@define{encoding}%
   \MT@permute@define{family}%
   \MT@permute@define{series}%
   \MT@permute@define{shape}%
   \MT@permute@define{size}%
   \edef\@tempa{\MT@tempencoding/%
                \MT@tempfamily/%
                \MT@tempseries/%
                \MT@tempshape/%
                \MT@tempsize}%
   \def\@tempb{////}%
   \ifx\@tempa\@tempb\else
      \ifx\MT@tempencoding\@empty
         \MT@warning{%
            You have to specify an encoding for \MT@permutelist. list\MessageBreak
            `\csname MT@\MT@permutelist @name\endcsname'. I will ignore it}%
      \else
         \MT@ifdefined@n{MT@\MT@permutelist @\@tempa}{%
            \MT@warning{\MT@permutelist. list
               `\csname MT@\MT@permutelist @name\endcsname' will override list\MessageBreak
               `\csname MT@\MT@permutelist @\@tempa\endcsname' for font `\@tempa'}%
         }{}%
         \ifx\MT@tempsize\@empty\else
            \expandafter\MT@size@check\@tempa//\@nil
         \fi
         \global\MT@edef@n{MT@\MT@permutelist @\@tempa}%
               {\csname MT@\MT@permutelist @name\endcsname}%
      \fi
   \fi
   \MT@increment\MT@cnt@size
   \MT@ifdefined@n{MT@tempsize\romannumeral\MT@cnt@size}%
      {\MT@permute@@@@@}{}%
}
\def\MT@size@check#1//#2\@nil{%
   \MT@ifempty{#2}{}{%
      \MT@let@nc{MT@tempsize\romannumeral\MT@cnt@size}\@undefined
      \edef\@tempa{\MT@tempencoding/\MT@tempfamily/\MT@tempseries/\MT@tempshape/}%
      \MT@warning{Size may only be specified if all other font\MessageBreak
         characteristics are specified, too. Ignoring size\MessageBreak
         in \MT@permutelist. list `\csname MT@\MT@permutelist @name\endcsname'}%
   }%
}
\def\MT@permute@define#1{%
   \expandafter\@tempcnta\csname MT@cnt@#1\endcsname
   \MT@ifdefined@n{MT@temp#1\romannumeral\@tempcnta}{%
      \MT@edef@n{MT@temp#1}{\csname MT@temp#1\romannumeral\@tempcnta\endcsname}%
   }{%
      \MT@let@nc{MT@temp#1}\@empty
   }%
}
\def\MT@permute@reset{%
   \MT@permute@reset@{encoding}%
   \MT@permute@reset@{family}%
   \MT@permute@reset@{series}%
   \MT@permute@reset@{shape}%
   \MT@permute@reset@{size}%
}
\def\MT@permute@reset@#1{%
   \@tempcnta\@ne
   \MT@loop
      \MT@let@nc{MT@temp#1\romannumeral\@tempcnta}\@undefined
      \advance\@tempcnta\@ne
      \MT@ifdefined@n{MT@temp#1\romannumeral\@tempcnta}
         {\@tempswatrue}
         {\@tempswafalse}%
      \if@tempswa\MT@repeat
}
\def\MT@capitalize#1#2\@nil{%
   \uppercase{\def\@tempb{#1}}%
   \edef\@tempb{\@tempb#2}}%
\def\microtypesetup{\setkeys{MTX}}
\def\MT@define@optionX#1{%
   \define@key{MTX}{#1}[true]{%
      \@for\MT@val:=##1\do{%
         \MT@capitalize#1\@nil
         \MT@remove@spaces{\MT@val}%
         \MT@ifempty{\MT@val}{}{%
            \@tempcnta\m@ne
            \def\@tempa{true}%
            \ifx\MT@val\@tempa
               \expandafter\expandafter\expandafter\ifx\expandafter
               \csname ifMT@#1\expandafter\endcsname\csname iftrue\endcsname
                  \expandafter\@tempcnta\csname MT@#1level\endcsname
                  \MT@info{\@tempb\space enabled}%
               \else
                  \MT@warning{You cannot enable #1 if it was disabled\MessageBreak
                              in the package options,}%
               \fi
               \let\MT@val\relax
            \fi
            \def\@tempa{false}%
            \ifx\MT@val\@tempa
               \@tempcnta\z@
               \MT@info{\@tempb\space disabled}%
               \let\MT@val\relax
            \fi
            \def\@tempa{compatibility}%
            \ifx\MT@val\@tempa
               \@tempcnta\@ne
               \MT@let@nc{MT@#1level}\@ne
               \MT@info{\@tempb\space set to level 1}%
               \let\MT@val\relax
            \fi
            \def\@tempa{nocompatibility}%
            \ifx\MT@val\@tempa
               \@tempcnta\tw@
               \MT@let@nc{MT@#1level}\tw@
               \MT@info{\@tempb\space set to level 2}%
               \let\MT@val\relax
            \fi
            \ifx\MT@val\relax\else
               \MT@warning{Value `\MT@val' not recognized}%
            \fi
            \ifnum\@tempcnta>\m@ne
               \def\@tempa{Expansion}%
               \ifx\@tempa\@tempb
                  \pdfadjustspacing\@tempcnta
               \else
                  \pdfprotrudechars\@tempcnta
               \fi
            \fi
         }%
      }%
   }%
}
\MT@define@optionX{protrusion}
\MT@define@optionX{expansion}
\define@key{MTX}{activate}[]{%
   \setkeys{MTX}{protrusion={#1}}%
   \setkeys{MTX}{expansion={#1}}%
}
\def\MT@gobblethree#1#2#3{}
\let\MT@saved@setupfont\MT@setupfont
\define@key{MTX}{disable}[]{%
   \MT@info{Inactivate microtype package}%
   \let\MT@setupfont\MT@gobblethree
}
\define@key{MTX}{enable}[]{%
   \MT@info{Reactivate microtype package}%
   \let\MT@setupfont\MT@saved@setupfont
}
\newif\ifMT@opt@protrusion
\newif\ifMT@opt@expansion
\newif\ifMT@opt@auto
\def\MT@define@option#1{%
   \define@key{MT}{#1}[true]{%
      \csname MT@opt@#1true\endcsname
      \@for\MT@val:=##1\do{%
         \MT@remove@spaces{\MT@val}%
         \MT@ifempty{\MT@val}{}{%
            \def\@tempa{false}%
            \ifx\MT@val\@tempa
               \csname MT@#1false\endcsname
               \let\MT@val\relax
            \fi
            \def\@tempa{compatibility}%
            \ifx\MT@val\@tempa
               \MT@def@n{MT@#1level}{1}%
               \let\MT@val\relax
            \fi
            \def\@tempa{nocompatibility}%
            \ifx\MT@val\@tempa
               \MT@def@n{MT@#1level}{2}%
               \let\MT@val\relax
            \fi
            \ifx\MT@val\relax\else
               \csname MT@#1true\endcsname
               \def\@tempa{true}%
               \ifx\MT@val\@tempa
               \else
                  \MT@ifdefined@n{MT@#1list@@\MT@val}{%
                     \global\MT@edef@n{MT@#1@setname}{\MT@val}%
                     \MT@info@nl{Using #1 set `\MT@val'}%
                  }{%
                     \global\MT@def@n{MT@#1@setname}{alltext}%
                     \MT@warning@nl{%
                        The #1 set `\MT@val' is undeclared.\MessageBreak
                        Using set `\csname MT@#1@setname\endcsname' instead}%
                  }%
               \fi
            \fi
         }%
      }%
   }%
}
\MT@define@option{protrusion}
\MT@define@option{expansion}
\define@key{MT}{activate}[]{%
   \setkeys{MT}{protrusion={#1}}%
   \setkeys{MT}{expansion={#1}}%
}
\define@key{MT}{DVIoutput}[true]{\csname MT@DVIoutput#1\endcsname}
\define@key{MT}{draft}[true]{\csname MT@draft#1\endcsname}
\define@key{MT}{final}[true]{%
   \def\@tempa{#1}\def\@tempb{true}%
   \ifx\@tempa\@tempb
      \MT@draftfalse
   \else
      \MT@drafttrue
   \fi}
\define@key{MT}{verbose}[true]{%
   \def\@tempa{#1}\def\@tempb{true}%
   \ifx\@tempa\@tempb
      \let\MT@vinfo\MT@info@nl
   \fi}
\define@key{MT}{auto}[true]{\csname MT@auto#1\endcsname\MT@opt@autotrue}
\define@key{MT}{selected}[true]{\csname MT@selected#1\endcsname}
\define@key{MT}{factor}[1000]{\MT@define@number\MT@prot@factor{#1}{factor}}
\define@key{MT}{stretch}[20]{\MT@define@number\MT@stretch{#1}{stretch}}
\define@key{MT}{shrink}[20]{\MT@define@number\MT@shrink{#1}{shrink}}
\define@key{MT}{step}[5]{\MT@define@number\MT@step{#1}{step}}
\def\MT@define@number#1#2#3{%
   \MT@ifnumber{#2}{%
      \def#1{#2 }%
   }{%
      \MT@warning@nl{Value `#2' for option `#3' is not a number.\MessageBreak
                     Using default value}%
   }%
}
\MT@protrusiontrue
\ifnum\pdfoutput=\z@\else
   \ifnum\MT@pdftex@no=4\relax
      \MT@expansiontrue
      \MT@autotrue
   \fi
\fi
\MT@info@nl{Trying to load local config file `microtype.cfg' ..}
\IfFileExists{microtype.cfg}{%
   \begingroup
   \MT@file@catcodes
   \input{microtype.cfg}%
   \endgroup
   \MT@info@nl{... local config file loaded successfully}%
}{%
   \MT@warning@nl{... local config file not found! This will\MessageBreak
                  almost certainly lead to undesired results}%
}
\def\ProcessOptionsWithKV#1{%
   \let\@tempc\relax
   \let\KVo@tempa\@empty
   \@for\CurrentOption:=\@classoptionslist\do{%
      \@ifundefined{KV@#1@\CurrentOption}{}{%
         \edef\KVo@tempa{\KVo@tempa,\CurrentOption,}%
         \@expandtwoargs\@removeelement\CurrentOption
            \@unusedoptionlist\@unusedoptionlist
      }%
   }%
   \edef\KVo@tempa{%
      \noexpand\setkeys{#1}{%
         \KVo@tempa\@ptionlist{\@currname.\@currext}%
      }%
   }%
   \KVo@tempa
   \AtEndOfPackage{\let\@unprocessedoptions\relax}%
   \let\CurrentOption\@empty
}
\ProcessOptionsWithKV{MT}
\ifMT@DVIoutput
   \ifnum\pdfoutput=\z@
      \MT@info@nl{Generating DVI output}
   \else
      \MT@info@nl{Changing output mode to DVI}
      \pdfoutput\z@
      \ifMT@opt@expansion\else
         \MT@expansionfalse
      \fi
   \fi
\else
   \MT@info@nl{Generating \ifnum\pdfoutput=\z@ DVI \else PDF \fi output}
\fi
\ifMT@draft
   \MT@info@nl{`draft' option active.\MessageBreak
               Disabling all micro-typographic features}
   \MT@protrusionfalse
   \MT@expansionfalse
   \let\MT@setupfont\relax
   \let\microtypesetup\@gobble
   \renewcommand{\UseMicroTypeSet}[2][]{}
   \renewcommand{\SetProtrusion}[3][]{}
   \renewcommand{\SetExpansion}[3][]{}
\else
   \ifMT@protrusion
      \MT@info@nl{Character protrusion enabled (level \MT@protrusionlevel)%
         \ifnum\MT@prot@factor=\@m\else,\MessageBreak factor: \MT@prot@factor\fi}
      \MT@ifdefined@n{MT@protrusion@setname}{}{%
         \global\def\MT@protrusion@setname{alltext}%
         \MT@info@nl{Using default protrusion set `alltext'}%
      }
   \else
      \MT@info@nl{No character protrusion}
   \fi
   \ifMT@expansion
      \ifnum\MT@stretch=\m@ne
         \def\MT@stretch{20 }
      \fi
      \ifnum\MT@shrink=\m@ne
         \ifnum\MT@stretch>\z@
            \let\MT@shrink\MT@stretch
         \else
            \def\MT@shrink{20 }
         \fi
      \fi
      \ifnum\MT@step=\m@ne
         \ifnum\MT@stretch>\MT@shrink
            \ifnum\MT@shrink=\z@
               \@tempcnta=\MT@stretch
            \else
               \@tempcnta=\MT@shrink
            \fi
         \else
            \ifnum\MT@stretch=\z@
               \@tempcnta=\MT@shrink
            \else
               \@tempcnta=\MT@stretch
            \fi
         \fi
         \divide\@tempcnta by 5\relax
      \else
         \@tempcnta=\MT@step
      \fi
      \ifnum\@tempcnta=\z@ \@tempcnta=\@ne\fi
      \edef\MT@step{\number\@tempcnta\space}
      \let\MT@auto\@empty
      \ifMT@auto
         \ifnum\MT@pdftex@no=4\relax
            \ifnum\pdfoutput=\z@
               \ifMT@opt@auto
                  \MT@warning@nl{%
                     Automatic font expansion only works for PDF output.\MessageBreak
                     However, you are creating a DVI file. I will switch\MessageBreak
                     automatic font expansion off and hope that expanded\MessageBreak
                     fonts are available}
               \fi
               \MT@autofalse
            \else
               \def\MT@auto{autoexpand}
            \fi
         \else
            \ifMT@opt@auto
               \MT@warning@nl{%
                  Your version of pdftex is too old for automatic\MessageBreak
                  font expansion. I will switch it off and hope that\MessageBreak
                  expanded fonts are available on your system.\MessageBreak
                  Install pdftex version 1.20a or newer}
            \fi
            \MT@autofalse
            \def\MT@auto{1000 }
         \fi
      \else
         \ifnum\MT@pdftex@no<4\relax
            \def\MT@auto{1000 }
         \fi
      \fi
      \MT@info@nl{\ifMT@auto Automatic f\else F\fi ont expansion enabled
                  (level \MT@expansionlevel),\MessageBreak
                  stretch: \MT@stretch/ shrink: \MT@shrink/ step: \MT@step/
                  \ifMT@selected\else non-\fi selected}
      \MT@ifdefined@n{MT@expansion@setname}{}{%
         \global\def\MT@expansion@setname{basictext}%
         \MT@info@nl{Using default expansion set `basictext'}%
      }
   \else
      \MT@info@nl{No font expansion}
   \fi
\fi
\ifMT@protrusion
   \pdfprotrudechars\MT@protrusionlevel
\fi
\ifMT@expansion
   \pdfadjustspacing\MT@expansionlevel
\fi
\endinput
%%
%% End of file `microtype.sty'.


==> Pruning via OT/nicefrac.tex <==
%%
%% This is file `nicefrac.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% units.dtx  (with options: `nicefrac')
%%
%% LaTeX package for typesetting nice fractions
%%
%% Copyright (C) 1998 Axel Reichert
%% See the files README and COPYING.
%%
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesPackage{nicefrac}[1998/08/04 v0.9b Nice fractions]
\newlength{\L@UnitsRaiseDisplaystyle}
\newlength{\L@UnitsRaiseTextstyle}
\newlength{\L@UnitsRaiseScriptstyle}
\RequirePackage{ifthen}
\DeclareRobustCommand*{\@UnitsNiceFrac}[3][]{%
  \ifthenelse{\boolean{mmode}}{%
    \settoheight{\L@UnitsRaiseDisplaystyle}{%
      \ensuremath{\displaystyle#1{M}}%
    }%
    \settoheight{\L@UnitsRaiseTextstyle}{%
      \ensuremath{\textstyle#1{M}}%
    }%
    \settoheight{\L@UnitsRaiseScriptstyle}{%
      \ensuremath{\scriptstyle#1{M}}%
    }%
    \settoheight{\@tempdima}{%
      \ensuremath{\scriptscriptstyle#1{M}}%
    }%
    \addtolength{\L@UnitsRaiseDisplaystyle}{%
      -\L@UnitsRaiseScriptstyle%
    }%
    \addtolength{\L@UnitsRaiseTextstyle}{%
      -\L@UnitsRaiseScriptstyle%
    }%
    \addtolength{\L@UnitsRaiseScriptstyle}{-\@tempdima}%
    \mathchoice
      {%
        \raisebox{\L@UnitsRaiseDisplaystyle}{%
          \ensuremath{\scriptstyle#1{#2}}%
        }%
      }%
      {%
        \raisebox{\L@UnitsRaiseTextstyle}{%
          \ensuremath{\scriptstyle#1{#2}}%
        }%
      }%
      {%
        \raisebox{\L@UnitsRaiseScriptstyle}{%
          \ensuremath{\scriptscriptstyle#1{#2}}%
        }%
      }%
      {%
        \raisebox{\L@UnitsRaiseScriptstyle}{%
          \ensuremath{\scriptscriptstyle#1{#2}}%
        }%
      }%
    \mkern-2mu/\mkern-1mu%
    \bgroup
      \mathchoice
        {\scriptstyle}%
        {\scriptstyle}%
        {\scriptscriptstyle}%
        {\scriptscriptstyle}%
      #1{#3}%
    \egroup
  }%
  {%
    \settoheight{\L@UnitsRaiseTextstyle}{#1{M}}%
    \settoheight{\@tempdima}{%
      \ensuremath{%
        \mbox{\fontsize\sf@size\z@\selectfont#1{M}}%
      }%
    }%
    \addtolength{\L@UnitsRaiseTextstyle}{-\@tempdima}%
    \raisebox{\L@UnitsRaiseTextstyle}{%
      \ensuremath{%
        \mbox{\fontsize\sf@size\z@\selectfont#1{#2}}%
      }%
    }%
    \ensuremath{\mkern-2mu}/\ensuremath{\mkern-1mu}%
    \ensuremath{%
      \mbox{\fontsize\sf@size\z@\selectfont#1{#3}}%
    }%
  }%
}
\DeclareRobustCommand*{\@UnitsUglyFrac}[3][]{%
  \ifthenelse{\boolean{mmode}}{%
    \frac{#1{#2}}{#1{#3}}%
  }%
  {%
    #1{#2}/#1{#3}%
    \PackageWarning{nicefrac}{%
      You used \protect\nicefrac\space or
      \protect\unitfrac\space in text mode\MessageBreak
      and specified the ``ugly'' option.\MessageBreak
      The fraction may be ambiguous or wrong.\MessageBreak
      Please make sure the denominator is
      correct.\MessageBreak
      If it is, you can safely ignore\MessageBreak
      this warning
    }%
  }%
}
\DeclareOption{nice}{%
  \DeclareRobustCommand*{\nicefrac}{\@UnitsNiceFrac}%
}
\DeclareOption{ugly}{%
  \DeclareRobustCommand*{\nicefrac}{\@UnitsUglyFrac}%
}
\ExecuteOptions{nice}
\ProcessOptions*
\endinput
%%
%% End of file `nicefrac.sty'.


==> algorithm.tex <==
%%%%%%%%%%%   ALGORITHMS STYLE  %%%%%%%%%%%
% This style defines an environment for algorithms with the following
% features:
%
% 1) Defines an Theorem like environment (not exactly one) for
%    algorithms called ``algorithm''.
%    \begin{algorithm}{NAME} ... \end{algorithm}
%    NAME is the NAME of the algorithm.
%    Algorithms are numbered using a counter called ``algorithm''.
%
% 2) Inside this environment, the following commands are defined.
%
%    \=  Put the small left arrow commonly used for assignment.
%
%    \invariant{INVARIANT} Use to describe invariants, put its parameter
%                          between ``{}'' in math mode.
%
%    \begin{Block} ... \end{Block} Environment use to start a indented
%                                  block of instructions \end{Block} put
%                                  an ``end'' to close the block.
%
%    \nextBlock{SEPARATOR} Inside a Block, it allows to put a separator
%                          of parts of the indented block. Usefull for
%                          constructions like ``IF..THEN..ELSE..END''
%                       i.e. If cond then
%                            \begin{Block}
%                               then part
%                            \nextBlock{else}
%                               else part
%                            \end{Block}
%
% 3) \Blockindent and \algorithmindent are length that specify the
%    indentention of Blocks and of the algorithm resp.
%
%   4) Instructions are separated by ``\\'', ``\par'' or by leaving a
%      blank line. Before an ``\end{Block}'' a ``\\'' can't be used.
%
%
% Created by Jose Alberto Fernandez R.
% e-mail:    alberto@cs.umd.edu
%

%
\newcounter{algorithm}
\newtheorem{Alg@orithm}[algorithm]{Algorithm}
% Invariants
\newcommand{\inv@ariant}[1]{\mbox{$\{#1\}$}}
% Steps environment
\newenvironment{ste@ps}[1]{
\begin{list}{}
{\setlength\labelsep{0in}
\addtolength\partopsep\topsep
\addtolength\partopsep\parsep
\setlength\parsep{0in}
\setlength\topsep{0in}
\setlength\itemsep{0in}
\setlength\labelwidth{0in}
\setlength\rightmargin{0in}
\setlength\leftmargin{#1}}
}{
\end{list}
}

% Block environment
% Indentation of the Block
\newlength{\Blockindent}
% NextBlock command
\newcommand{\next@Block}[1]{
\end{ste@ps}
#1
\begin{ste@ps}{\Blockindent}
\item
}

\newenvironment{Blo@ck}{
\let\nextBlock\next@Block
\begin{ste@ps}{\Blockindent}
\item
}{
\end{ste@ps}
end
}
% Algorithm environment
% Assign command
\newcommand{\ass@ign}{\mbox{$\leftarrow$}}
% Indentation of the algorithm
\newlength{\algorithmindent}
% Algorithm definition
\newenvironment{algorithm}[1]{
\let\=\ass@ign
\let\invariant\inv@ariant
\let\Block\Blo@ck
\let\endBlock\endBlo@ck
\begin{Alg@orithm} #1
\rm\par
\begin{ste@ps}{\algorithmindent}
\item
}{
\end{ste@ps}
\bf end
\end{Alg@orithm}
}

% Setting default indentation
\setlength{\algorithmindent}{1em}
\setlength{\Blockindent}{2em}

% End of algorithm.sty


==> microtype.tex <==
%%
%% This is file `microtype.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% microtype.dtx  (with options: `package')
%%
%% -----------------------------------------------------------------------
%%                        The `microtype' package
%%        An interface to the micro-typographic extensions of pdfTeX
%%           Copyright (c) 2004, 2005 R Schlicht <w.m.l@gmx.net>
%%
%% This work  may be  distributed and/or modified  under the conditions of
%% the LaTeX Project Public License, either version 1.3 of this license or
%% (at your option) any later version.  The latest version of this license
%% is in:  http://www.latex-project.org/lppl.txt, and version 1.3 or later
%% is part of all distributions of LaTeX version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of the files microtype.dtx and microtype.ins and the
%% derived file microtype.sty.
%%
%% -----------------------------------------------------------------------
%%
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{microtype}
      [2005/02/02 v1.6a Micro-typography with pdfTeX (RS)]
\RequirePackage{keyval}[1997/11/10]
\def\MT@info{\PackageInfo{microtype}}
\def\MT@info@nl#1{\MT@info{#1\@gobble}}
\let\MT@vinfo\@gobble
\def\MT@warning{\PackageWarning{microtype}}
\def\MT@warning@nl#1{\MT@warning{#1\@gobble}}
\def\MT@error{\PackageError{microtype}}
\newcommand{\DeclareMicroTypeSet}[3][]{}
\newcommand{\UseMicroTypeSet}[2][]{}
\newcommand{\DeclareMicroTypeAlias}[2]{}
\newcommand{\SetProtrusion}[3][]{}
\newcommand{\SetExpansion}[3][]{}
\newcommand{\DeclareCharacterInheritance}[3][]{}
\newcommand{\microtypesetup}[1]{}
\def\DeclareMicroTypeSet{%
   \@ifstar
      {\@ifnextchar[\MT@DeclareSet{\MT@DeclareSet[]}}%
      {\@ifnextchar[\MT@DeclareSet{\MT@DeclareSet[]}}%
}
\def\MT@DeclareSet[#1]#2#3{}
\@onlypreamble{\DeclareMicroTypeSet}
\@onlypreamble{\UseMicroTypeSet}
\@onlypreamble{\DeclareMicroTypeAlias}
\let\MT@pdftex@no\z@
\ifx\pdftexversion\@undefined \else
   \ifx\pdftexversion\relax \else
      \def\MT@pdftex@no{4}
      \ifnum\pdftexversion < 120
         \let\MT@pdftex@no\thr@@
         \ifnum\pdftexversion = 14
            \ifnum \expandafter`\pdftexrevision < `h
               \let\MT@pdftex@no\tw@
            \fi
            \ifnum \expandafter`\pdftexrevision < `f
               \let\MT@pdftex@no\@ne
            \fi
         \else
            \ifnum\pdftexversion < 14
               \let\MT@pdftex@no\@ne
            \fi
         \fi
      \fi
   \fi
\fi
\let\MT@exitornot\relax
\ifnum\MT@pdftex@no<\tw@
   \def\MT@exitornot{%
      \AtEndOfPackage{\let\@unprocessedoptions\relax}%
      \let\CurrentOption\@empty
      \endinput
   }
   \MT@warning@nl{%
      \ifcase\MT@pdftex@no
         You don't seem to be using pdftex.\MessageBreak
      \or
         You are using a pdftex version older than 0.14f.\MessageBreak
         microtype doesn't support such antiquated versions.\MessageBreak
         Please install a newer version of pdftex.\MessageBreak
      \fi
         All micro-typographic features will be disabled%
   }
\fi
\MT@exitornot
\def\MT@catcodes{%
   \@makeother\-%
   \@makeother\,%
   \@makeother\/%
   \@makeother\`%
   \@makeother\'%
   \@makeother\"%
   \catcode`\^7\relax
}
\def\MT@restore@catcodes#1{%
   \ifx\relax#1\else
      \noexpand\catcode`\noexpand#1\the\catcode`#1\relax
      \expandafter\MT@restore@catcodes
   \fi
}
\edef\MT@restore@catcodes{%
   \MT@restore@catcodes\-\,\/\`\'\"\^\relax
}
\MT@catcodes
\AtEndOfPackage{\MT@restore@catcodes}
\AtBeginDocument{%
   \@ifpackageloaded{pdfcprot}{%
      \MT@error{%
         Detected the `pdfcprot' package!\MessageBreak
         `microtype' and `pdfcprot' may not be used together}%
         {The `pdfcprot' package provides an interface to
          character protrusion.\MessageBreak
          So does the `microtype' package.
          Using both packages at the same\MessageBreak
          time will almost certainly lead to undesired results.
          Have your choice!}%
   }{}%
}
\expandafter\ifx\the\font\nullfont\normalfont\fi
\newif\ifMT@DVIoutput
\newif\ifMT@draft
\newif\ifMT@protrusion
\newif\ifMT@expansion
\newif\ifMT@auto
\newif\ifMT@selected
\def\MT@expansionlevel{2}
\def\MT@protrusionlevel{2}
\let\MT@stretch\m@ne
\let\MT@shrink\m@ne
\let\MT@step\m@ne
\let\MT@prot@factor\@m
\def\MT@def@n#1{\expandafter\def\csname #1\endcsname}
\def\MT@edef@n#1{\expandafter\edef\csname #1\endcsname}
\def\MT@let@nc#1{\expandafter\let\csname #1\endcsname}
\def\MT@let@cn#1#2{\expandafter\let\expandafter#1\csname #2\endcsname}
\def\MT@hop@else@fi#1\else#2\fi{\fi#1}
\ifx\ifdefined\@undefined\MT@hop@else@fi
   \def\MT@ifdefined@c#1{%
      \ifx#1\@undefined
         \expandafter\@secondoftwo
      \else
         \expandafter\@firstoftwo
      \fi
   }
   \def\MT@ifdefined@n#1{%
      \expandafter\ifx\csname#1\endcsname\relax
         \expandafter\@secondoftwo
      \else
         \expandafter\@firstoftwo
      \fi
   }
\else
   \def\MT@ifdefined@c#1{%
      \ifdefined#1%
         \expandafter\@firstoftwo
      \else
         \expandafter\@secondoftwo
      \fi
   }
   \def\MT@ifdefined@n#1{%
      \ifcsname#1\endcsname
         \expandafter\@firstoftwo
      \else
         \expandafter\@secondoftwo
      \fi
   }
\fi
\begingroup
\catcode`\%=12\relax
\catcode`\&=14\relax
\gdef\MT@ifempty#1{&
  \if %#1%&
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}
\endgroup
\def\MT@ifnumber#1{%
   \if!\ifnum9<1#1!\else_\fi
      \expandafter\@firstoftwo
   \else
      \expandafter\@secondoftwo
   \fi
}
\def\MT@xadd#1#2{%
   \expandafter\ifx#1\relax
      \xdef#1{#2}%
   \else
      \begingroup
         \edef\x{#2}%
         \toks@=\expandafter\expandafter\expandafter{\expandafter#1\x}%
         \xdef#1{\the\toks@}%
      \endgroup
   \fi
}
\newif\ifMT@inlist@
\def\MT@in@list#1#2{%
   \MT@inlist@false
   \def\MT@given{#1}%
   \def\MT@lt##1{%
      \def\MT@next{##1}\ifx\MT@next\MT@given\MT@inlist@true\fi}#2%
}
\let\MT@lt\@empty
\def\MT@in@llist#1#2{%
   \MT@inlist@false
   \def\MT@in@l##1#1,##2\@nil{%
      \ifx\\##2\\\else
         \MT@inlist@true
      \fi}%
   \expandafter\MT@in@l#2,#1,\@nil
}
\def\MT@loop#1\MT@repeat{%
   \def\MT@iterate{#1\relax\expandafter\MT@iterate\fi}%
   \MT@iterate \let\MT@iterate\relax}
\let\MT@repeat\fi
\newcount\MT@count
\def\MT@increment#1{%
   \MT@count#1\relax
   \advance\MT@count \@ne
   \edef#1{\number\MT@count}%
}
\def\MT@remove@spaces#1{\expandafter\KV@@sp@def\expandafter#1\expandafter{#1}}
\def\MT@setupfont{%
   \ifx\MT@vinfo\MT@info@nl
      \MT@info{Setting up font `\expandafter\string\font@name'}\fi
   \expandafter\expandafter\expandafter
      \MT@split@name\expandafter\string\font@name\@nil
   \MT@find@file{\MT@family}%
   \ifx\MT@familyalias\@empty\else\MT@find@file{\MT@familyalias}\fi
   \ifx\f@encoding\cf@encoding\else\@@enc@update\fi
   \MT@checkfor{protrusion}%
   \ifMT@font@protrusion
      \MT@set@prot@codes
   \else
      \MT@vinfo{... No protrusion}%
   \fi
   \MT@checkfor{expansion}%
   \ifMT@font@expansion
      \MT@set@exp@codes
   \else
      \MT@vinfo{... No expansion}%
   \fi
}
\newif\ifMT@font@protrusion
\newif\ifMT@font@expansion
\def\MT@checkfor#1{%
   \csname ifMT@#1\endcsname
      \csname MT@font@#1true\endcsname
      \MT@checklist{#1}{encoding}%
      \MT@checklist@family{#1}%
      \MT@checklist{#1}{series}%
      \MT@checklist{#1}{shape}%
      \MT@checklist{#1}{size}%
   \fi
}
\def\MT@checklist#1#2{%
   \csname ifMT@font@#1\endcsname\MT@checklist@{#1}{#2}\fi
}
\def\MT@checklist@#1#2{%
   \edef\@tempa{\csname MT@#1@setname\endcsname}%
   \MT@ifdefined@n{MT@#1list@#2@\@tempa}{%
      \def\MT@listname{\csname MT@#1list@#2@\@tempa\endcsname}%
      \expandafter\expandafter\expandafter\MT@in@list
         \expandafter\expandafter\expandafter
            {\csname MT@#2\endcsname}\MT@listname
      \ifMT@inlist@
      \else
         \csname MT@font@#1false\endcsname
      \fi
   }{%
   }%
}
\def\MT@checklist@family#1{%
   \csname ifMT@font@#1\endcsname\MT@checklist@family@{#1}\fi
}
\def\MT@checklist@family@#1{%
   \MT@checklist@{#1}{family}%
   \csname ifMT@font@#1\endcsname\else
      \ifx\MT@familyalias\@empty\else
         \edef\@tempa{\csname MT@#1@setname\endcsname}%
         \def\MT@listname{\csname MT@#1list@family@\@tempa\endcsname}%
         \expandafter\expandafter\expandafter\MT@in@list
            \expandafter
               {\MT@familyalias}\MT@listname
         \ifMT@inlist@
            \csname MT@font@#1true\endcsname
         \fi
      \fi
   \fi
}
\def\MT@split@name#1/#2/#3/#4/#5\@nil{%
   \gdef\MT@encoding{#1}%
   \gdef\MT@family{#2}%
   \gdef\MT@series{#3}%
   \gdef\MT@shape{#4}%
   \gdef\MT@size{#5}%
   \global\let\MT@familyalias\@empty
   \MT@ifdefined@n{MT@\MT@family @alias}{%
      \MT@escapechar{\csname MT@\MT@family @alias\endcsname}%
      \global\let\MT@familyalias\MT@val
   }{}%
}
\def\MT@set@prot@codes{%
   \MT@get@codes@list{prot}%
   \MT@ifdefined@n{MT@protcodes@\MT@protcodes@name}{%
      \MT@get@factor
      \MT@get@inh@list{protrusion}%
      \MT@ifdefined@c\MT@protrusioninh@name{%
         \MT@let@cn\@tempc{MT@protrusioninh@\MT@protrusioninh@name}%
            \ifx\@tempc\@empty\else
               \let\MT@inh@name\MT@protrusioninh@name
               \expandafter\MT@inhdo\@tempc,\relax,%
            \fi
         \global\MT@let@nc{MT@protrusioninh@\MT@protrusioninh@name}\@empty
      }{}%
      \MT@load@list{prot}{\MT@protcodes@name}%
      \MT@let@cn\@tempc{MT@protcodes@\MT@protcodes@name}%
      \expandafter\MT@protdo\@tempc,\relax,%
   }{}%
}
\def\MT@protdo#1,{%
   \ifx\relax#1\@empty\else
      \MT@protsplit #1==\relax
      \expandafter\MT@protdo\fi
}
\def\MT@protsplit#1=#2=#3\relax{%
   \KV@@sp@def\@tempa{#1}%
   \ifx\@tempa\@empty\else
      \MT@get@slot
      \ifnum\MT@char > \m@ne
         \KV@@sp@def\@tempb{#2}%
         \expandafter\MT@protsplit@val\@tempb\relax
      \fi
   \fi
}
\def\MT@protsplit@val#1,#2\relax{%
   \KV@@sp@def\@tempb{#1}%
   \MT@ifempty{\@tempb}{}{%
      \MT@adjustprotcode
      \lpcode\font@name\MT@char=\@tempcntb
   }%
   \KV@@sp@def\@tempb{#2}%
   \MT@ifempty{\@tempb}{}{%
      \MT@adjustprotcode
      \rpcode\font@name\MT@char=\@tempcntb
   }%
   \MT@ifdefined@c\MT@protrusioninh@name{%
      \MT@ifdefined@n{MT@inh@\MT@protrusioninh@name @\MT@char @}{%
         \MT@set@prot@children
      }{}%
   }{}%
}
\ifnum\MT@pdftex@no>\tw@
   \def\MT@adjustprotcode{%
      \MT@get@charwd
      \multiply\@tempcntb \@tempb
      \ifnum\@tempcntb=\z@ \else
         \divide\@tempcntb \fontdimen6 \font@name
         \MT@adjustprotcode@
      \fi
   }
   \MT@ifdefined@c\fontcharwd{%
      \def\MT@get@charwd{%
         \@tempcntb=\number\fontcharwd\font@name\MT@char}%
   }{%
      \def\MT@get@charwd{%
         \setbox\z@=\hbox{\font@name \char\MT@char}%
         \@tempcntb=\wd\z@}%
   }
\else
   \def\MT@adjustprotcode{%
      \@tempcntb=\@tempb
      \ifnum\@tempcntb=\z@ \else
         \MT@adjustprotcode@
      \fi
   }
\fi
\def\MT@adjustprotcode@{%
   \multiply\@tempcntb \MT@prot@factor@
   \divide\@tempcntb \@m
   \ifnum\@tempcntb > \@m
      \MT@warning@nl{Protrusion factor \@tempb\space for character
         `\@tempa'\MessageBreak too large (= \the\@tempcntb) in
         protrusion list `\MT@protcodes@name'}%
   \else
      \ifnum\@tempcntb < -\@m
         \MT@warning@nl{Protrusion factor \@tempb\space for character
            `\@tempa'\MessageBreak too small (= \the\@tempcntb) in
            protrusion list `\MT@protcodes@name'}%
      \fi
   \fi
}
\def\MT@set@prot@children{%
   \def\MT@lt##1{%
      \lpcode\font@name##1=\lpcode\font@name\MT@char
      \rpcode\font@name##1=\rpcode\font@name\MT@char
   }%
   \csname MT@inh@\MT@protrusioninh@name @\MT@char @\endcsname
}
\def\MT@get@factor{%
   \MT@ifdefined@n{MT@protcodes@\MT@protcodes@name @factor}{%
      \MT@let@cn\MT@prot@factor@{MT@protcodes@\MT@protcodes@name @factor}%
      \MT@vinfo{... ... Multiplying protrusion factors by \MT@prot@factor@/1000}%
   }{%
      \let\MT@prot@factor@\MT@prot@factor
   }%
}
\newif\ifMT@selected@exp
\def\MT@set@exp@codes{%
   \ifMT@selected
      \MT@get@codes@list{exp}%
      \MT@ifdefined@n{MT@expcodes@\MT@expcodes@name}{%
         \MT@get@extraopt
         \MT@resetefcode
         \MT@get@inh@list{expansion}%
         \MT@ifdefined@c\MT@expansioninh@name{%
            \MT@let@cn\@tempc{MT@expansioninh@\MT@expansioninh@name}%
               \ifx\@tempc\@empty\else
                  \let\MT@inh@name\MT@expansioninh@name
                  \expandafter\MT@inhdo\@tempc,\relax,%
               \fi
            \global\MT@let@nc{MT@expansioninh@\MT@expansioninh@name}\@empty
         }{}%
         \MT@load@list{exp}{\MT@expcodes@name}%
         \MT@let@cn\@tempc{MT@expcodes@\MT@expcodes@name}%
         \expandafter\MT@expdo\@tempc,\relax,%
         \pdffontexpand\font@name \MT@stretch@ \MT@shrink@ \MT@step@ \MT@auto@
      }{}%
   \else
      \MT@selected@exptrue
      \MT@get@codes@list{exp}%
      \MT@ifdefined@n{MT@expcodes@\MT@expcodes@name}{%
         \MT@get@extraopt
      }{%
         \let\MT@exp@factor@\@m
         \let\MT@stretch@\MT@stretch
         \let\MT@shrink@\MT@shrink
         \let\MT@step@\MT@step
         \let\MT@auto@\MT@auto
      }%
      \MT@resetefcode
      \pdffontexpand\font@name \MT@stretch@ \MT@shrink@ \MT@step@ \MT@auto@
   \fi
}
\def\MT@resetefcode@{%
   \@tempcnta\z@
   \MT@loop
      \efcode\font@name\@tempcnta=\MT@exp@factor@
      \advance\@tempcnta \@ne
      \ifnum\@tempcnta < \@cclvi \MT@repeat
}
\ifnum\MT@pdftex@no<4
   \let\MT@resetefcode\MT@resetefcode@
\else
   \def\MT@resetefcode{%
      \ifnum\MT@exp@factor@=\@m \else
         \MT@resetefcode@
      \fi
   }
\fi
\def\MT@expdo#1,{%
   \ifx\relax#1\@empty\else
      \MT@expsplit #1==\relax
      \expandafter\MT@expdo\fi
}
\def\MT@expsplit#1=#2=#3\relax{%
   \KV@@sp@def\@tempa{#1}%
   \ifx\@tempa\@empty\else
      \MT@get@slot
      \ifnum\MT@char > \m@ne
         \KV@@sp@def\@tempb{#2}%
         \@tempcnta=\@tempb
         \multiply\@tempcnta \MT@exp@factor@
         \divide\@tempcnta \@m
         \efcode\font@name\MT@char=\@tempcnta
         \MT@ifdefined@c\MT@expansioninh@name{%
            \MT@ifdefined@n{MT@inh@\MT@expansioninh@name @\MT@char @}%
               {\MT@set@exp@children}{}%
         }{}%
      \fi
   \fi
}
\def\MT@set@exp@children{%
   \def\MT@lt##1{%
      \efcode\font@name##1=\efcode\font@name\MT@char
   }%
   \csname MT@inh@\MT@expansioninh@name @\MT@char @\endcsname
}
\def\MT@get@extraopt{%
   \MT@ifdefined@n{MT@expcodes@\MT@expcodes@name @factor}{%
      \MT@let@cn\MT@exp@factor@{MT@expcodes@\MT@expcodes@name @factor}%
      \MT@vinfo{... ... Multiplying expansion factors by \MT@exp@factor@/1000}%
   }{%
      \let\MT@exp@factor@\@m
   }%
   \MT@ifdefined@n{MT@expcodes@\MT@expcodes@name @stretch}{%
      \MT@let@cn\MT@stretch@{MT@expcodes@\MT@expcodes@name @stretch}%
      \MT@vinfo{... ... Setting stretch factor to \MT@stretch@}%
   }{%
      \let\MT@stretch@\MT@stretch
   }%
   \MT@ifdefined@n{MT@expcodes@\MT@expcodes@name @shrink}{%
      \MT@let@cn\MT@shrink@{MT@expcodes@\MT@expcodes@name @shrink}%
      \MT@vinfo{... ... Setting shrink factor to \MT@shrink@}%
   }{%
      \let\MT@shrink@\MT@shrink
   }%
   \MT@ifdefined@n{MT@expcodes@\MT@expcodes@name @step}{%
      \MT@let@cn\MT@step@{MT@expcodes@\MT@expcodes@name @step}%
      \MT@vinfo{... ... Setting step factor to \MT@step@}%
   }{%
      \let\MT@step@\MT@step
   }%
   \MT@ifdefined@n{MT@expcodes@\MT@expcodes@name @auto}{%
      \MT@let@cn\MT@auto@{MT@expcodes@\MT@expcodes@name @auto}%
      \MT@vinfo{... ... Setting automatic expansion to \MT@auto@}%
   }{%
      \let\MT@auto@\MT@auto
   }%
}
\def\MT@load@list#1#2{%
   \edef\@tempa{#2}%
   \MT@let@cn\@tempb{MT@#1codes@\@tempa load}%
   \ifx\@tempa\@tempb
      \MT@warning{#1. list `\@tempa' cannot load itself}%
   \else
      \ifx\@tempb\relax\else
         \MT@ifdefined@n{MT@#1codes@\@tempb}{%
            \MT@vinfo{... ... Additionally loading #1. list `\@tempb'}%
            \begingroup
               \MT@load@list{#1}{\@tempb}%
            \endgroup
            \MT@let@cn\@tempc{MT@#1codes@\@tempb}%
            \expandafter\csname MT@#1do\expandafter\endcsname\@tempc,\relax,%
         }{%
            \MT@warning{%
               #1. list `\@tempb' undefined. Cannot load it\MessageBreak
               from list `\@tempa'}%
         }%
      \fi
   \fi
}
\let\MT@file@list\@empty
\def\MT@find@file#1{%
   \expandafter\MT@in@llist\expandafter
         {\csname MT@file@#1\endcsname}\MT@file@list
   \ifMT@inlist@\else
      \begingroup
      \MT@file@catcodes
      \InputIfFileExists{mt-#1.cfg}{%
         \MT@xadd\MT@file@list{\csname MT@file@#1\endcsname,}%
         \MT@vinfo{... Loading font settings from mt-#1.cfg}%
      }{%
         \expandafter\MT@get@basefamily#1\relax\relax\relax
         \expandafter\MT@in@llist\expandafter
                {\csname MT@file@\@tempa\endcsname}\MT@file@list
         \ifMT@inlist@\else
            \InputIfFileExists{mt-\@tempa.cfg}{%
               \MT@xadd\MT@file@list{\csname MT@file@\@tempa\endcsname,}%
               \MT@vinfo{... Loading font settings from mt-\@tempa.cfg}%
            }{%
               \MT@xadd\MT@file@list{\csname MT@file@#1\endcsname,}%
               \MT@vinfo{... No file mt-#1.cfg}%
            }%
         \fi
      }%
      \endgroup
   \fi
}
\def\MT@file@catcodes{%
     \makeatletter
     \catcode`\ 9%
     \catcode`\^7%
     \catcode`\^^I9%
     \catcode`\^^M9%
     \catcode`\\\z@
     \catcode`\{\@ne
     \catcode`\}\tw@
     \catcode`\#6%
     \catcode`\%14%
   \@makeother\<%
   \@makeother\>%
   \@makeother\*%
   \@makeother\.%
   \@makeother\-%
   \@makeother\/%
   \@makeother\[%
   \@makeother\]%
   \@makeother\`%
   \@makeother\'%
   \@makeother\"%
   \@makeother\&%
   \@makeother\;%
   \@makeother\,%
   \@makeother\!%
   \@makeother\?%
   \@makeother\$%
   \@makeother\_%
   \@makeother\~%
   \@makeother\=%
}
\def\MT@get@basefamily#1#2#3#4\relax{%
   \ifx\relax#2\relax\def\@tempa{#1}\else
      \ifx\relax#3\relax\def\@tempa{#1#2}\else
         \def\@tempa{#1#2#3}%
         \ifx\relax#4\relax\else
            \edef\@tempc{\string#4}%
            \edef\@tempb{\string x}%
            \ifx\@tempc\@tempb\else
               \edef\@tempb{\string j}%
               \ifx\@tempc\@tempb\else
                  \edef\@tempb{\string w}%
                  \ifx\@tempc\@tempb\else
                     \def\@tempa{#1#2#3#4}%
                  \fi
               \fi
            \fi
         \fi
      \fi
   \fi
}
\def\MT@get@listname#1{%
   \def\@tempb{#1}%
   \MT@next@listname1111\relax
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \MT@next@listname1110\relax
   }%
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \MT@next@listname1100\relax
   }%
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \MT@next@listname1010\relax
   }%
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \MT@next@listname1000\relax
   }%
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \MT@next@listname0100\relax
   }%
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \MT@next@listname0010\relax
   }%
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \MT@next@listname0000\relax
   }%
}
\def\MT@next@listname#1#2#3#4{%
   \edef\@tempa{\MT@encoding/%
                \ifnum#1=\@ne \MT@family\fi/%
                \ifnum#2=\@ne \MT@series\fi/%
                \ifnum#3=\@ne \MT@shape\fi/%
                \ifnum#4=\@ne \MT@size\fi}%
   \MT@ifdefined@n{MT@\@tempb @\@tempa}{}{%
      \ifnum#1=\@ne
         \ifx\MT@familyalias\@empty\else
            \edef\@tempa{\MT@encoding/%
                         \MT@familyalias/%
                         \ifnum#2=\@ne \MT@series\fi/%
                         \ifnum#3=\@ne \MT@shape\fi/%
                         \ifnum#4=\@ne \MT@size\fi}%
         \fi
      \fi
   }%
}
\def\MT@get@codes@list#1{%
   \MT@get@listname{#1codes}%
   \MT@ifdefined@n{MT@#1codes@\@tempa}{%
      \global\MT@edef@n{MT@#1codes@name}{\csname MT@#1codes@\@tempa\endcsname}%
      \ifMT@selected@exp
         \MT@vinfo{... Applying non-selected expansion (list `\MT@expcodes@name')}%
      \else
         \MT@vinfo{... Using #1. list `\csname MT@#1codes@name\endcsname'}%
      \fi
   }{%
      \global\MT@let@nc{MT@#1codes@\csname MT@#1codes@name\endcsname}\@undefined
      \ifMT@selected@exp
         \MT@vinfo{... Applying non-selected expansion}%
      \else
         \MT@warning{I cannot find a #1. list for
                     `\expandafter\string\font@name'.\MessageBreak
                     Switching off #1. for this font}%
       \fi
   }%
}
\def\MT@get@inh@list#1{%
   \MT@get@listname{#1inh}%
   \MT@ifdefined@n{MT@#1inh@\@tempa}{%
      \MT@edef@n{MT@#1inh@name}{\csname MT@#1inh@\@tempa\endcsname}%
   }{%
      \MT@let@nc{MT@#1inh@name}\@undefined
   }%
}
\begingroup
   \catcode`\/=0
   /catcode`/\=12
   /catcode`/"=12
   /catcode`/A=12
   /catcode`/C=12
   /catcode`/E=12
   /catcode`/H=12
   /catcode`/L=12
   /catcode`/R=12
   /catcode`/T=12
   /lowercase{%
      /def/x{%
         /def/Mt@letterstring{THE LETTER}%
         /def/Mt@isaletter ##1THE LETTER##2##3/relax{%
            /@tempswafalse
            /ifx/relax##1/relax
               /@tempswatrue
               /edef/Mt@char{/number`##2}%
               /Mt@testrest{/Mt@letterstring}{##3}%
            /fi
         }%
         /def/Mt@characterstring{THE CHARACTER}%
         /def/Mt@isacharacter ##1THE CHARACTER##2##3/relax{%
            /@tempswafalse
            /ifx/relax##1/relax
               /@tempswatrue
               /edef/Mt@char{/number`##2}%
               /Mt@testrest{/Mt@characterstring}{##3}%
            /fi
         }%
         /def/Mt@charstring{\CHAR"}%
         /def/Mt@isachar##1\CHAR"##2##3##4/relax{%
            /@tempswafalse
            /ifx/relax##1/relax
               /@tempswatrue
               /if##3\/relax
                  /edef/Mt@char{/number"##2}%
                  /Mt@testrest{/Mt@charstring}{##3##4}%
               /else
                  /edef/Mt@char{/number"##2##3}%
                  /Mt@testrest{/Mt@charstring}{##4}%
               /fi
            /fi
         }%
      }%
   }
/expandafter/endgroup/x
\def\Mt@testrest#1#2{%
   \edef\x{#1}%
   \edef\y{#2}%
   \ifx\x\y\else
      \def\Mt@rest{#2}%
   \fi
}
\def\MT@get@slot{%
   \MT@count=\escapechar
   \escapechar=`\\
   \let\Mt@rest\@empty
   \let\Mt@char\m@ne
   \edef\MT@char{\expandafter\meaning\@tempa}%
   \expandafter\expandafter\expandafter\Mt@isaletter
         \expandafter\MT@char\Mt@letterstring \relax\relax
   \ifnum\Mt@char < \z@
      \expandafter\expandafter\expandafter\Mt@isacharacter
            \expandafter\MT@char\Mt@characterstring \relax\relax
      \if@tempswa
         \expandafter\MT@get@number\@tempa\relax\relax
      \fi
      \ifnum\Mt@char < \z@
         \expandafter\ifx\expandafter\ \@tempa\relax
            \edef\Mt@char{\number`\\}%
         \else
            \edef\MT@char{\expandafter\csname\expandafter\MT@encoding
                              \expandafter\string\@tempa\endcsname}%
            \edef\MT@char{\expandafter\meaning\MT@char}%
            \expandafter\expandafter\expandafter\Mt@isachar
                  \expandafter\MT@char\Mt@charstring \relax\relax\relax
            \if@tempswa \else
               \expandafter\expandafter\expandafter\Mt@isaletter
                     \expandafter\MT@char\Mt@letterstring \relax\relax
            \fi
         \fi
         \ifnum\Mt@char < \z@
            \expandafter\MT@two@tokens\@tempa\relax\relax
            \edef\MT@char{\expandafter\meaning\@tempa}%
            \expandafter\expandafter\expandafter\Mt@isaletter
                  \expandafter\MT@char\Mt@letterstring \relax\relax
            \if@tempswa \else
               \MT@warning{Unknown slot number of `\@tempa' in\MessageBreak
                           encoding `\MT@encoding'. Ignoring it}%
            \fi
         \fi
      \fi
   \fi
   \ifx\Mt@rest\@empty\else
      \MT@warning{Unknown slot number of `\@tempa' in\MessageBreak
                  encoding `\MT@encoding'.
                  Make sure it's a single character\MessageBreak
                  (or a number). Ignoring it}%
      \let\Mt@char\m@ne
   \fi
   \let\MT@char\Mt@char
   \escapechar=\MT@count
}
\def\MT@two@tokens#1#2\relax{%
   \MT@ifempty{#2}{}%
      {\edef\@tempa{\@tempa}}%
}
\def\MT@get@number#1#2#3\relax{%
   \ifx\relax#3\relax\else
      \ifx\relax#2\relax\else
         \if#1"\relax
            \def\@tempc{\uppercase{\edef\Mt@char{\number#1#2#3}}}%
            \@tempc
         \else
            \if#1'\relax
               \def\Mt@char{\number#1#2#3}%
            \else
               \MT@ifnumber{#1#2#3}{%
                  \def\Mt@char{\number#1#2#3}%
               }{}%
            \fi
         \fi
         \ifnum\Mt@char > \@cclv
            \MT@warning{%
               Number \noexpand#1\noexpand#2\noexpand#3 in encoding
               `\MT@encoding' too large!\MessageBreak Ignoring it}%
            \let\Mt@char\m@ne
         \fi
         \let\Mt@rest\@empty
      \fi
   \fi
}
\let\MT@font@list\@empty
\g@addto@macro\pickup@font{%
   \begingroup \escapechar\m@ne
   \expandafter\MT@in@llist\expandafter
         {\font@name}\MT@font@list
   \ifMT@inlist@\else
      \MT@setupfont
      \xdef\MT@font@list{\MT@font@list\font@name,}%
   \fi
   \endgroup
}
\let\MT@pickupfont\pickup@font
\AtBeginDocument{%
   \ifx\MT@pickupfont\pickup@font\else
      \MT@warning@nl{%
         Another package has overwritten the definition\MessageBreak
         of \string\pickup@font. I might not be able to\MessageBreak
         apply any micro-typography. Please find the\MessageBreak
         culprit, and load it before the microtype package}%
   \fi
}
\def\DeclareMicroTypeSet{%
   \@ifstar
      {\@ifnextchar[%]
         \MT@DeclareSetAndUseIt
         {\MT@DeclareSetAndUseIt[]}}%
      {\@ifnextchar[%]
         \MT@DeclareSet
         {\MT@DeclareSet[]}}%
}
\def\MT@DeclareSet[#1]#2#3{%
   \MT@DeclareSet@{#1}{#2}{#3}%
}
\def\MT@DeclareSetAndUseIt[#1]#2#3{%
   \MT@DeclareSet@{#1}{#2}{#3}%
   \UseMicroTypeSet[#1]{#2}%
}
\def\MT@DeclareSet@#1#2#3{%
  \KV@@sp@def\@tempa{#1}%
  \MT@ifempty{\@tempa}{%
     \MT@declare@sets{protrusion}{#2}{#3}%
     \MT@declare@sets{expansion} {#2}{#3}%
  }{%
     \expandafter\MT@declare@sets\expandafter{\@tempa}{#2}{#3}%
  }%
}
\let\MT@tmp@setname\@empty
\def\MT@declare@sets#1#2#3{%
   \KV@@sp@def\MT@tmp@setname{#2}%
   \global\MT@let@nc{MT@#1list@@\MT@tmp@setname}\@empty
   \setkeys{MT#1@set}{#3}%
}
\def\MT@define@set@keys#1{%
   \MT@define@set@key{#1}{encoding}%
   \MT@define@set@key{#1}{family}%
   \MT@define@set@key{#1}{series}%
   \MT@define@set@key{#1}{shape}%
   \MT@define@set@key@size{#1}%
}
\def\MT@define@set@key#1#2{%
   \define@key{MT#1@set}{#2}[]{%
      \@for\MT@val:=##1\do{%
         \MT@remove@spaces{\MT@val}%
         \MT@get@highlevel{#2}%
         \MT@escapechar{\MT@val}%
         \MT@addto@list{#1}{#2}{\MT@val}%
      }%
   }%
}
\def\MT@get@highlevel#1{%
   \MT@getlast{\MT@val}%
   \if*\@tempb
      \MT@ifempty{\@tempa}{\def\@tempa{#1}}{}%
      \def\MT@val{\csname \@tempa default\endcsname}%
      \ifx\@nodocument\relax\else
         \expandafter\ifx
               \csname MT@check@\MT@tmp@setname @\@tempa\endcsname\@empty
         \else
            \global\MT@edef@n{MT@\MT@tmp@setname @\@tempa @default}{\MT@val}%
            \edef\x{{\MT@tmp@setname}{\@tempa}}%
            \expandafter\AtBeginDocument\expandafter{%
               \expandafter\MT@check@default\x
            }%
            \global\MT@let@nc{MT@check@\MT@tmp@setname @\@tempa}\@empty
         \fi
      \fi
   \fi
}
\def\MT@check@default#1#2{%
   \MT@let@cn\@tempa{MT@#1@#2@default}%
   \edef\@tempb{\csname #2default\endcsname}%
   \ifx\@tempa\@tempb\else
      \MT@warning@nl{\expandafter\noexpand\csname #2default\endcsname
            has changed (`\@tempa' <> `\@tempb')!\MessageBreak
            This might affect the `#1' font set.\MessageBreak
            Please make all relevant font changes *before*\MessageBreak
            loading the `microtype' package}%
   \fi
}
\def\MT@getlast#1{\def\@tempa{}\def\@tempb{}%
   \expandafter\MT@getlast@#1\@nil}
\def\MT@getlast@#1{\ifx#1\@nil \let\next=\relax
   \else \edef\@tempa{\@tempa\@tempb}\def\@tempb{#1}%
      \let\next=\MT@getlast@\fi \next}
\def\MT@escapechar#1{%
   \begingroup
   \escapechar\m@ne
   \xdef\MT@val{\expandafter\string\csname #1\endcsname}%
   \endgroup
}
\def\MT@define@set@key@size#1{%
   \define@key{MT#1@set}{size}[]{%
      \@for\MT@val:=##1\do{%
         \MT@remove@spaces{\MT@val}%
         \MT@get@size
         \MT@addto@list{#1}{size}{\MT@val}%
      }%
   }%
}
\def\MT@get@size{%
   \let\@tempa\relax
   \if*\MT@val\relax
      \def\@tempa{\normalsize}%
   \else
      \MT@let@cn\@tempa{\MT@val}%
   \fi
   \ifx\@tempa\relax\else
      \begingroup
         \def\set@fontsize##1##2##3##4\@nil{\gdef\MT@val{##2}}%
         \@tempa\@nil
      \endgroup
   \fi
   \setbox\z@=\hbox{\MT@count=0\MT@val\relax
      \ifnum\MT@count=\z@
         \@tempswafalse
      \else
         \@tempswatrue
      \fi\expandafter}%
   \if@tempswa
      \@defaultunits\@tempdima\MT@val pt\relax\@nnil
      \edef\MT@val{\strip@pt\@tempdima}%
   \else
      \MT@warning{Could not parse font size `\MT@val'\MessageBreak
                  in font set `\MT@tmp@setname'}%
   \fi
}
\def\MT@addto@list#1#2#3{%
   \expandafter\MT@xadd\csname MT@#1list@#2@\MT@tmp@setname\endcsname
      {\noexpand\MT@lt{#3}}%
}
\MT@define@set@keys{protrusion}
\MT@define@set@keys{expansion}
\renewcommand{\UseMicroTypeSet}[2][]{%
   \KV@@sp@def\@tempa{#1}%
   \MT@ifempty{\@tempa}{%
      \MT@use@sets{protrusion}{#2}%
      \MT@use@sets{expansion} {#2}%
   }{%
      \expandafter\MT@use@sets\expandafter{\@tempa}{#2}%
   }%
}
\def\MT@use@sets#1#2{%
   \KV@@sp@def{\@tempa}{#2}%
   \MT@ifdefined@n{MT@#1list@@\@tempa}{%
      \global\MT@edef@n{MT@#1@setname}{\@tempa}%
      \MT@info{Using #1 set `\@tempa'}%
   }{%
      \MT@ifdefined@n{MT@#1@setname}{}{%
         \global\MT@def@n{MT@#1@setname}{alltext}%
      }%
      \MT@warning{The #1 set `\@tempa' is undeclared.\MessageBreak
                  Using set `\csname MT@#1@setname\endcsname' instead}%
   }%
}
\renewcommand{\DeclareMicroTypeAlias}[2]{%
   \KV@@sp@def\@tempa{#1}%
   \KV@@sp@def\@tempb{#2}%
   \global\MT@edef@n{MT@\@tempa @alias}{\@tempb}%
}
\renewcommand{\SetProtrusion}[3][]{%
   \global\let\MT@protcodes@name\@undefined
   \let\MT@load\@undefined
   \let\MT@extra@factor\@undefined
   \setkeys{MT@protcodes}{#1}%
   \MT@get@codes@name{prot}%
   \MT@set@factor
   \global\MT@def@n{MT@protcodes@\MT@protcodes@name}{#3}%
   \setkeys{MT@protcodes}{#2}%
   \def\MT@permutelist{protcodes}%
   \MT@permute
}
\renewcommand{\SetExpansion}[3][]{%
   \global\let\MT@expcodes@name\@undefined
   \let\MT@extra@factor\@undefined
   \let\MT@extra@stretch\@undefined
   \let\MT@extra@shrink\@undefined
   \let\MT@extra@step\@undefined
   \let\MT@extra@auto\@undefined
   \let\MT@load\@undefined
   \setkeys{MT@expcodes}{#1}%
   \MT@get@codes@name{exp}%
   \MT@set@exp@opt
   \global\MT@def@n{MT@expcodes@\MT@expcodes@name}{#3}%
   \setkeys{MT@expcodes}{#2}%
   \def\MT@permutelist{expcodes}%
   \MT@permute
}
\def\MT@get@codes@name#1{%
   \MT@ifdefined@n{MT@#1codes@name}{%
      \MT@ifdefined@n{MT@#1codes@\csname MT@#1codes@name\endcsname}{%
         \MT@warning{Redefining list `\csname MT@#1codes@name\endcsname'}%
      }{}%
   }{%
      \@tempcnta=\@ne
      \MT@loop
         \MT@ifdefined@n{MT@#1codes@#1-\romannumeral\@tempcnta}{%
            \advance \@tempcnta \@ne
         }{%
            \global\MT@edef@n{MT@#1codes@name}{#1-\romannumeral\@tempcnta}%
            \@tempcnta=\z@
         }%
         \ifnum\@tempcnta > \z@ \MT@repeat
   }%
   \MT@ifdefined@c\MT@load{%
      \global\MT@let@nc{MT@#1codes@\csname MT@#1codes@name\endcsname load}\MT@load
   }{}%
}
\def\MT@set@factor{%
   \MT@ifdefined@c\MT@extra@factor{%
      \global\MT@let@nc{MT@protcodes@\MT@protcodes@name @factor}\MT@extra@factor
   }{}%
}
\def\MT@set@exp@opt{%
   \MT@ifdefined@c\MT@extra@factor{%
      \global\MT@let@nc{MT@expcodes@\MT@expcodes@name @factor}\MT@extra@factor
   }{}%
   \MT@ifdefined@c\MT@extra@stretch{%
      \global\MT@let@nc{MT@expcodes@\MT@expcodes@name @stretch}\MT@extra@stretch
   }{}%
   \MT@ifdefined@c\MT@extra@shrink{%
      \global\MT@let@nc{MT@expcodes@\MT@expcodes@name @shrink}\MT@extra@shrink
   }{}%
   \MT@ifdefined@c\MT@extra@step{%
      \global\MT@let@nc{MT@expcodes@\MT@expcodes@name @step}\MT@extra@step
   }{}%
   \MT@ifdefined@c\MT@extra@auto{%
      \global\MT@let@nc{MT@expcodes@\MT@expcodes@name @auto}\MT@extra@auto
   }{}%
}
\def\MT@define@code@key#1#2{%
   \define@key{MT@#1}{#2}[]{%
      \@tempcnta=\@ne
      \@for\MT@val:=##1\do{%
         \MT@remove@spaces{\MT@val}%
         \MT@get@highlevel{#2}%
         \MT@edef@n{MT@temp#2\romannumeral\@tempcnta}{\MT@val}%
         \advance\@tempcnta \@ne
      }%
   }%
}
\def\MT@define@code@key@size#1{%
   \define@key{MT@#1}{size}[]{%
      \@tempcnta=\@ne
      \@for\MT@val:=##1\do{%
         \MT@remove@spaces{\MT@val}%
         \MT@get@size
         \MT@edef@n{MT@tempsize\romannumeral\@tempcnta}{\MT@val}%
         \advance\@tempcnta \@ne
      }%
   }%
}
\def\MT@declare@codes#1{%
   \define@key{MT@#1codes}{name}[]{%
      \MT@ifempty{##1}{}{%
         \global\MT@def@n{MT@#1codes@name}{##1}%
      }%
   }%
   \define@key{MT@#1codes}{load}[]{%
      \MT@ifempty{##1}{}{%
         \def\MT@load{##1}%
      }%
   }%
   \define@key{MT@#1codes}{factor}[]{%
      \MT@ifempty{##1}{}{%
         \def\MT@extra@factor{##1 }%
      }%
   }%
   \MT@define@code@key{#1codes}{encoding}%
   \MT@define@code@key{#1codes}{family}%
   \MT@define@code@key{#1codes}{series}%
   \MT@define@code@key{#1codes}{shape}%
   \MT@define@code@key@size{#1codes}%
}
\MT@declare@codes{prot}
\MT@declare@codes{exp}
\def\MT@define@expcodes@key#1{%
   \define@key{MT@expcodes}{#1}[]{%
      \MT@ifempty{##1}{}{%
         \MT@def@n{MT@extra@#1}{##1 }%
      }%
   }%
}
\MT@define@expcodes@key{stretch}
\MT@define@expcodes@key{shrink}
\MT@define@expcodes@key{step}
\define@key{MT@expcodes}{auto}[]{%
   \MT@ifempty{#1}{\def\@tempb{true}}{\def\@tempb{#1}}%
   \csname if\@tempb\endcsname
      \def\MT@extra@auto{autoexpand }%
   \else
      \let\MT@extra@auto\@empty
   \fi
}
\renewcommand{\DeclareCharacterInheritance}[3][]{%
   \KV@@sp@def\@tempa{#1}%
   \MT@ifempty{\@tempa}{%
       \MT@declare@char@inh{protrusion}{#2}{#3}%
       \MT@declare@char@inh{expansion} {#2}{#3}%
   }{%
       \expandafter\MT@declare@char@inh\expandafter{\@tempa}{#2}{#3}%
   }%
}
\def\MT@declare@char@inh#1#2#3{%
   \MT@let@nc{MT@#1inh@name}\@undefined
   \MT@get@inh@name{#1}%
   \global\MT@def@n{MT@#1inh@\csname MT@#1inh@name\endcsname}{#3}%
   \setkeys{MT@#1inh}{#2}%
   \def\MT@permutelist{#1inh}%
   \MT@permute
}
\def\MT@get@inh@name#1{%
   \@tempcnta=\@ne
   \MT@loop
      \MT@ifdefined@n{MT@#1inh@#1-inh-\romannumeral\@tempcnta}{%
         \advance \@tempcnta \@ne
      }{%
         \MT@edef@n{MT@#1inh@name}{#1-inh-\romannumeral\@tempcnta}%
         \@tempcnta=\z@
      }%
      \ifnum\@tempcnta > \z@ \MT@repeat
}
\def\MT@define@inh@key@encoding#1{%
   \define@key{MT@#1}{encoding}[]{%
      \KV@@sp@def\MT@val{##1}%
      \expandafter\MT@encoding@check\MT@val,\@nil
      \MT@get@highlevel{encoding}%
      \MT@edef@n{MT@tempencoding\romannumeral1}{\MT@val}%
   }%
}
\def\MT@encoding@check#1,#2\@nil{%
   \MT@ifempty{#2}{}{%
      \edef\MT@val{#1}%
      \MT@warning{You may only specify one encoding for character\MessageBreak
                  inheritance lists. Ignoring encoding #2}%
   }%
}
\def\MT@define@inh@keys#1{%
   \MT@define@inh@key@encoding{#1inh}%
   \MT@define@code@key{#1inh}{family}%
   \MT@define@code@key{#1inh}{series}%
   \MT@define@code@key{#1inh}{shape}%
   \MT@define@code@key@size{#1inh}%
}
\MT@define@inh@keys{protrusion}
\MT@define@inh@keys{expansion}
\def\MT@inhdo#1,{%
   \ifx\relax#1\@empty\else
      \MT@inhsplit #1==\relax
      \expandafter\MT@inhdo\fi
}
\def\MT@inhsplit#1=#2=#3\relax{%
   \KV@@sp@def\@tempa{#1}%
   \ifx\@tempa\@empty\else
      \MT@get@slot
      \ifnum\MT@char > \m@ne
         \let\MT@val\MT@char
         \let\MT@lt\relax
         \KV@@sp@def\@tempb{#2}%
         \@for\@tempa:=\@tempb\do{%
            \MT@remove@spaces{\@tempa}%
            \ifx\@tempa\@empty\else
               \MT@get@slot
               \ifnum\MT@char > \m@ne
                  \expandafter\MT@xadd\csname MT@inh@\MT@inh@name @\MT@val @\endcsname
                     {\noexpand\MT@lt{\MT@char}}%
               \fi
            \fi
         }%
      \fi
   \fi
}
\def\MT@permute{%
   \let\MT@cnt@encoding\@ne
   \MT@permute@
   \MT@permute@reset
}
\def\MT@permute@{%
   \let\MT@cnt@family\@ne
   \MT@permute@@
   \MT@increment\MT@cnt@encoding
   \MT@ifdefined@n{MT@tempencoding\romannumeral\MT@cnt@encoding}%
      {\MT@permute@}{}%
}
\def\MT@permute@@{%
   \let\MT@cnt@series\@ne
   \MT@permute@@@
   \MT@increment\MT@cnt@family
   \MT@ifdefined@n{MT@tempfamily\romannumeral\MT@cnt@family}%
      {\MT@permute@@}{}%
}
\def\MT@permute@@@{%
   \let\MT@cnt@shape\@ne
   \MT@permute@@@@
   \MT@increment\MT@cnt@series
   \MT@ifdefined@n{MT@tempseries\romannumeral\MT@cnt@series}%
      {\MT@permute@@@}{}%
}
\def\MT@permute@@@@{%
   \let\MT@cnt@size\@ne
   \MT@permute@@@@@
   \MT@increment\MT@cnt@shape
   \MT@ifdefined@n{MT@tempshape\romannumeral\MT@cnt@shape}%
      {\MT@permute@@@@}{}%
}
\def\MT@permute@@@@@{%
   \MT@permute@define{encoding}%
   \MT@permute@define{family}%
   \MT@permute@define{series}%
   \MT@permute@define{shape}%
   \MT@permute@define{size}%
   \edef\@tempa{\MT@tempencoding/%
                \MT@tempfamily/%
                \MT@tempseries/%
                \MT@tempshape/%
                \MT@tempsize}%
   \def\@tempb{////}%
   \ifx\@tempa\@tempb\else
      \ifx\MT@tempencoding\@empty
         \MT@warning{%
            You have to specify an encoding for \MT@permutelist. list\MessageBreak
            `\csname MT@\MT@permutelist @name\endcsname'. I will ignore it}%
      \else
         \MT@ifdefined@n{MT@\MT@permutelist @\@tempa}{%
            \MT@warning{\MT@permutelist. list
               `\csname MT@\MT@permutelist @name\endcsname' will override list\MessageBreak
               `\csname MT@\MT@permutelist @\@tempa\endcsname' for font `\@tempa'}%
         }{}%
         \ifx\MT@tempsize\@empty\else
            \expandafter\MT@size@check\@tempa//\@nil
         \fi
         \global\MT@edef@n{MT@\MT@permutelist @\@tempa}%
               {\csname MT@\MT@permutelist @name\endcsname}%
      \fi
   \fi
   \MT@increment\MT@cnt@size
   \MT@ifdefined@n{MT@tempsize\romannumeral\MT@cnt@size}%
      {\MT@permute@@@@@}{}%
}
\def\MT@size@check#1//#2\@nil{%
   \MT@ifempty{#2}{}{%
      \MT@let@nc{MT@tempsize\romannumeral\MT@cnt@size}\@undefined
      \edef\@tempa{\MT@tempencoding/\MT@tempfamily/\MT@tempseries/\MT@tempshape/}%
      \MT@warning{Size may only be specified if all other font\MessageBreak
         characteristics are specified, too. Ignoring size\MessageBreak
         in \MT@permutelist. list `\csname MT@\MT@permutelist @name\endcsname'}%
   }%
}
\def\MT@permute@define#1{%
   \expandafter\@tempcnta\csname MT@cnt@#1\endcsname
   \MT@ifdefined@n{MT@temp#1\romannumeral\@tempcnta}{%
      \MT@edef@n{MT@temp#1}{\csname MT@temp#1\romannumeral\@tempcnta\endcsname}%
   }{%
      \MT@let@nc{MT@temp#1}\@empty
   }%
}
\def\MT@permute@reset{%
   \MT@permute@reset@{encoding}%
   \MT@permute@reset@{family}%
   \MT@permute@reset@{series}%
   \MT@permute@reset@{shape}%
   \MT@permute@reset@{size}%
}
\def\MT@permute@reset@#1{%
   \@tempcnta\@ne
   \MT@loop
      \MT@let@nc{MT@temp#1\romannumeral\@tempcnta}\@undefined
      \advance\@tempcnta\@ne
      \MT@ifdefined@n{MT@temp#1\romannumeral\@tempcnta}
         {\@tempswatrue}
         {\@tempswafalse}%
      \if@tempswa\MT@repeat
}
\def\MT@capitalize#1#2\@nil{%
   \uppercase{\def\@tempb{#1}}%
   \edef\@tempb{\@tempb#2}}%
\def\microtypesetup{\setkeys{MTX}}
\def\MT@define@optionX#1{%
   \define@key{MTX}{#1}[true]{%
      \@for\MT@val:=##1\do{%
         \MT@capitalize#1\@nil
         \MT@remove@spaces{\MT@val}%
         \MT@ifempty{\MT@val}{}{%
            \@tempcnta\m@ne
            \def\@tempa{true}%
            \ifx\MT@val\@tempa
               \expandafter\expandafter\expandafter\ifx\expandafter
               \csname ifMT@#1\expandafter\endcsname\csname iftrue\endcsname
                  \expandafter\@tempcnta\csname MT@#1level\endcsname
                  \MT@info{\@tempb\space enabled}%
               \else
                  \MT@warning{You cannot enable #1 if it was disabled\MessageBreak
                              in the package options,}%
               \fi
               \let\MT@val\relax
            \fi
            \def\@tempa{false}%
            \ifx\MT@val\@tempa
               \@tempcnta\z@
               \MT@info{\@tempb\space disabled}%
               \let\MT@val\relax
            \fi
            \def\@tempa{compatibility}%
            \ifx\MT@val\@tempa
               \@tempcnta\@ne
               \MT@let@nc{MT@#1level}\@ne
               \MT@info{\@tempb\space set to level 1}%
               \let\MT@val\relax
            \fi
            \def\@tempa{nocompatibility}%
            \ifx\MT@val\@tempa
               \@tempcnta\tw@
               \MT@let@nc{MT@#1level}\tw@
               \MT@info{\@tempb\space set to level 2}%
               \let\MT@val\relax
            \fi
            \ifx\MT@val\relax\else
               \MT@warning{Value `\MT@val' not recognized}%
            \fi
            \ifnum\@tempcnta>\m@ne
               \def\@tempa{Expansion}%
               \ifx\@tempa\@tempb
                  \pdfadjustspacing\@tempcnta
               \else
                  \pdfprotrudechars\@tempcnta
               \fi
            \fi
         }%
      }%
   }%
}
\MT@define@optionX{protrusion}
\MT@define@optionX{expansion}
\define@key{MTX}{activate}[]{%
   \setkeys{MTX}{protrusion={#1}}%
   \setkeys{MTX}{expansion={#1}}%
}
\def\MT@gobblethree#1#2#3{}
\let\MT@saved@setupfont\MT@setupfont
\define@key{MTX}{disable}[]{%
   \MT@info{Inactivate microtype package}%
   \let\MT@setupfont\MT@gobblethree
}
\define@key{MTX}{enable}[]{%
   \MT@info{Reactivate microtype package}%
   \let\MT@setupfont\MT@saved@setupfont
}
\newif\ifMT@opt@protrusion
\newif\ifMT@opt@expansion
\newif\ifMT@opt@auto
\def\MT@define@option#1{%
   \define@key{MT}{#1}[true]{%
      \csname MT@opt@#1true\endcsname
      \@for\MT@val:=##1\do{%
         \MT@remove@spaces{\MT@val}%
         \MT@ifempty{\MT@val}{}{%
            \def\@tempa{false}%
            \ifx\MT@val\@tempa
               \csname MT@#1false\endcsname
               \let\MT@val\relax
            \fi
            \def\@tempa{compatibility}%
            \ifx\MT@val\@tempa
               \MT@def@n{MT@#1level}{1}%
               \let\MT@val\relax
            \fi
            \def\@tempa{nocompatibility}%
            \ifx\MT@val\@tempa
               \MT@def@n{MT@#1level}{2}%
               \let\MT@val\relax
            \fi
            \ifx\MT@val\relax\else
               \csname MT@#1true\endcsname
               \def\@tempa{true}%
               \ifx\MT@val\@tempa
               \else
                  \MT@ifdefined@n{MT@#1list@@\MT@val}{%
                     \global\MT@edef@n{MT@#1@setname}{\MT@val}%
                     \MT@info@nl{Using #1 set `\MT@val'}%
                  }{%
                     \global\MT@def@n{MT@#1@setname}{alltext}%
                     \MT@warning@nl{%
                        The #1 set `\MT@val' is undeclared.\MessageBreak
                        Using set `\csname MT@#1@setname\endcsname' instead}%
                  }%
               \fi
            \fi
         }%
      }%
   }%
}
\MT@define@option{protrusion}
\MT@define@option{expansion}
\define@key{MT}{activate}[]{%
   \setkeys{MT}{protrusion={#1}}%
   \setkeys{MT}{expansion={#1}}%
}
\define@key{MT}{DVIoutput}[true]{\csname MT@DVIoutput#1\endcsname}
\define@key{MT}{draft}[true]{\csname MT@draft#1\endcsname}
\define@key{MT}{final}[true]{%
   \def\@tempa{#1}\def\@tempb{true}%
   \ifx\@tempa\@tempb
      \MT@draftfalse
   \else
      \MT@drafttrue
   \fi}
\define@key{MT}{verbose}[true]{%
   \def\@tempa{#1}\def\@tempb{true}%
   \ifx\@tempa\@tempb
      \let\MT@vinfo\MT@info@nl
   \fi}
\define@key{MT}{auto}[true]{\csname MT@auto#1\endcsname\MT@opt@autotrue}
\define@key{MT}{selected}[true]{\csname MT@selected#1\endcsname}
\define@key{MT}{factor}[1000]{\MT@define@number\MT@prot@factor{#1}{factor}}
\define@key{MT}{stretch}[20]{\MT@define@number\MT@stretch{#1}{stretch}}
\define@key{MT}{shrink}[20]{\MT@define@number\MT@shrink{#1}{shrink}}
\define@key{MT}{step}[5]{\MT@define@number\MT@step{#1}{step}}
\def\MT@define@number#1#2#3{%
   \MT@ifnumber{#2}{%
      \def#1{#2 }%
   }{%
      \MT@warning@nl{Value `#2' for option `#3' is not a number.\MessageBreak
                     Using default value}%
   }%
}
\MT@protrusiontrue
\ifnum\pdfoutput=\z@\else
   \ifnum\MT@pdftex@no=4\relax
      \MT@expansiontrue
      \MT@autotrue
   \fi
\fi
\MT@info@nl{Trying to load local config file `microtype.cfg' ..}
\IfFileExists{microtype.cfg}{%
   \begingroup
   \MT@file@catcodes
   \input{microtype.cfg}%
   \endgroup
   \MT@info@nl{... local config file loaded successfully}%
}{%
   \MT@warning@nl{... local config file not found! This will\MessageBreak
                  almost certainly lead to undesired results}%
}
\def\ProcessOptionsWithKV#1{%
   \let\@tempc\relax
   \let\KVo@tempa\@empty
   \@for\CurrentOption:=\@classoptionslist\do{%
      \@ifundefined{KV@#1@\CurrentOption}{}{%
         \edef\KVo@tempa{\KVo@tempa,\CurrentOption,}%
         \@expandtwoargs\@removeelement\CurrentOption
            \@unusedoptionlist\@unusedoptionlist
      }%
   }%
   \edef\KVo@tempa{%
      \noexpand\setkeys{#1}{%
         \KVo@tempa\@ptionlist{\@currname.\@currext}%
      }%
   }%
   \KVo@tempa
   \AtEndOfPackage{\let\@unprocessedoptions\relax}%
   \let\CurrentOption\@empty
}
\ProcessOptionsWithKV{MT}
\ifMT@DVIoutput
   \ifnum\pdfoutput=\z@
      \MT@info@nl{Generating DVI output}
   \else
      \MT@info@nl{Changing output mode to DVI}
      \pdfoutput\z@
      \ifMT@opt@expansion\else
         \MT@expansionfalse
      \fi
   \fi
\else
   \MT@info@nl{Generating \ifnum\pdfoutput=\z@ DVI \else PDF \fi output}
\fi
\ifMT@draft
   \MT@info@nl{`draft' option active.\MessageBreak
               Disabling all micro-typographic features}
   \MT@protrusionfalse
   \MT@expansionfalse
   \let\MT@setupfont\relax
   \let\microtypesetup\@gobble
   \renewcommand{\UseMicroTypeSet}[2][]{}
   \renewcommand{\SetProtrusion}[3][]{}
   \renewcommand{\SetExpansion}[3][]{}
\else
   \ifMT@protrusion
      \MT@info@nl{Character protrusion enabled (level \MT@protrusionlevel)%
         \ifnum\MT@prot@factor=\@m\else,\MessageBreak factor: \MT@prot@factor\fi}
      \MT@ifdefined@n{MT@protrusion@setname}{}{%
         \global\def\MT@protrusion@setname{alltext}%
         \MT@info@nl{Using default protrusion set `alltext'}%
      }
   \else
      \MT@info@nl{No character protrusion}
   \fi
   \ifMT@expansion
      \ifnum\MT@stretch=\m@ne
         \def\MT@stretch{20 }
      \fi
      \ifnum\MT@shrink=\m@ne
         \ifnum\MT@stretch>\z@
            \let\MT@shrink\MT@stretch
         \else
            \def\MT@shrink{20 }
         \fi
      \fi
      \ifnum\MT@step=\m@ne
         \ifnum\MT@stretch>\MT@shrink
            \ifnum\MT@shrink=\z@
               \@tempcnta=\MT@stretch
            \else
               \@tempcnta=\MT@shrink
            \fi
         \else
            \ifnum\MT@stretch=\z@
               \@tempcnta=\MT@shrink
            \else
               \@tempcnta=\MT@stretch
            \fi
         \fi
         \divide\@tempcnta by 5\relax
      \else
         \@tempcnta=\MT@step
      \fi
      \ifnum\@tempcnta=\z@ \@tempcnta=\@ne\fi
      \edef\MT@step{\number\@tempcnta\space}
      \let\MT@auto\@empty
      \ifMT@auto
         \ifnum\MT@pdftex@no=4\relax
            \ifnum\pdfoutput=\z@
               \ifMT@opt@auto
                  \MT@warning@nl{%
                     Automatic font expansion only works for PDF output.\MessageBreak
                     However, you are creating a DVI file. I will switch\MessageBreak
                     automatic font expansion off and hope that expanded\MessageBreak
                     fonts are available}
               \fi
               \MT@autofalse
            \else
               \def\MT@auto{autoexpand}
            \fi
         \else
            \ifMT@opt@auto
               \MT@warning@nl{%
                  Your version of pdftex is too old for automatic\MessageBreak
                  font expansion. I will switch it off and hope that\MessageBreak
                  expanded fonts are available on your system.\MessageBreak
                  Install pdftex version 1.20a or newer}
            \fi
            \MT@autofalse
            \def\MT@auto{1000 }
         \fi
      \else
         \ifnum\MT@pdftex@no<4\relax
            \def\MT@auto{1000 }
         \fi
      \fi
      \MT@info@nl{\ifMT@auto Automatic f\else F\fi ont expansion enabled
                  (level \MT@expansionlevel),\MessageBreak
                  stretch: \MT@stretch/ shrink: \MT@shrink/ step: \MT@step/
                  \ifMT@selected\else non-\fi selected}
      \MT@ifdefined@n{MT@expansion@setname}{}{%
         \global\def\MT@expansion@setname{basictext}%
         \MT@info@nl{Using default expansion set `basictext'}%
      }
   \else
      \MT@info@nl{No font expansion}
   \fi
\fi
\ifMT@protrusion
   \pdfprotrudechars\MT@protrusionlevel
\fi
\ifMT@expansion
   \pdfadjustspacing\MT@expansionlevel
\fi
\endinput
%%
%% End of file `microtype.sty'.


==> nicefrac.tex <==
%%
%% This is file `nicefrac.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% units.dtx  (with options: `nicefrac')
%%
%% LaTeX package for typesetting nice fractions
%%
%% Copyright (C) 1998 Axel Reichert
%% See the files README and COPYING.
%%
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesPackage{nicefrac}[1998/08/04 v0.9b Nice fractions]
\newlength{\L@UnitsRaiseDisplaystyle}
\newlength{\L@UnitsRaiseTextstyle}
\newlength{\L@UnitsRaiseScriptstyle}
\RequirePackage{ifthen}
\DeclareRobustCommand*{\@UnitsNiceFrac}[3][]{%
  \ifthenelse{\boolean{mmode}}{%
    \settoheight{\L@UnitsRaiseDisplaystyle}{%
      \ensuremath{\displaystyle#1{M}}%
    }%
    \settoheight{\L@UnitsRaiseTextstyle}{%
      \ensuremath{\textstyle#1{M}}%
    }%
    \settoheight{\L@UnitsRaiseScriptstyle}{%
      \ensuremath{\scriptstyle#1{M}}%
    }%
    \settoheight{\@tempdima}{%
      \ensuremath{\scriptscriptstyle#1{M}}%
    }%
    \addtolength{\L@UnitsRaiseDisplaystyle}{%
      -\L@UnitsRaiseScriptstyle%
    }%
    \addtolength{\L@UnitsRaiseTextstyle}{%
      -\L@UnitsRaiseScriptstyle%
    }%
    \addtolength{\L@UnitsRaiseScriptstyle}{-\@tempdima}%
    \mathchoice
      {%
        \raisebox{\L@UnitsRaiseDisplaystyle}{%
          \ensuremath{\scriptstyle#1{#2}}%
        }%
      }%
      {%
        \raisebox{\L@UnitsRaiseTextstyle}{%
          \ensuremath{\scriptstyle#1{#2}}%
        }%
      }%
      {%
        \raisebox{\L@UnitsRaiseScriptstyle}{%
          \ensuremath{\scriptscriptstyle#1{#2}}%
        }%
      }%
      {%
        \raisebox{\L@UnitsRaiseScriptstyle}{%
          \ensuremath{\scriptscriptstyle#1{#2}}%
        }%
      }%
    \mkern-2mu/\mkern-1mu%
    \bgroup
      \mathchoice
        {\scriptstyle}%
        {\scriptstyle}%
        {\scriptscriptstyle}%
        {\scriptscriptstyle}%
      #1{#3}%
    \egroup
  }%
  {%
    \settoheight{\L@UnitsRaiseTextstyle}{#1{M}}%
    \settoheight{\@tempdima}{%
      \ensuremath{%
        \mbox{\fontsize\sf@size\z@\selectfont#1{M}}%
      }%
    }%
    \addtolength{\L@UnitsRaiseTextstyle}{-\@tempdima}%
    \raisebox{\L@UnitsRaiseTextstyle}{%
      \ensuremath{%
        \mbox{\fontsize\sf@size\z@\selectfont#1{#2}}%
      }%
    }%
    \ensuremath{\mkern-2mu}/\ensuremath{\mkern-1mu}%
    \ensuremath{%
      \mbox{\fontsize\sf@size\z@\selectfont#1{#3}}%
    }%
  }%
}
\DeclareRobustCommand*{\@UnitsUglyFrac}[3][]{%
  \ifthenelse{\boolean{mmode}}{%
    \frac{#1{#2}}{#1{#3}}%
  }%
  {%
    #1{#2}/#1{#3}%
    \PackageWarning{nicefrac}{%
      You used \protect\nicefrac\space or
      \protect\unitfrac\space in text mode\MessageBreak
      and specified the ``ugly'' option.\MessageBreak
      The fraction may be ambiguous or wrong.\MessageBreak
      Please make sure the denominator is
      correct.\MessageBreak
      If it is, you can safely ignore\MessageBreak
      this warning
    }%
  }%
}
\DeclareOption{nice}{%
  \DeclareRobustCommand*{\nicefrac}{\@UnitsNiceFrac}%
}
\DeclareOption{ugly}{%
  \DeclareRobustCommand*{\nicefrac}{\@UnitsUglyFrac}%
}
\ExecuteOptions{nice}
\ProcessOptions*
\endinput
%%
%% End of file `nicefrac.sty'.

